LEMURS: Learning Distributed Multi-Robot Interactions

This paper presents LEMURS, an algorithm for learning scalable multi-robot control policies from cooperative task demonstrations. We propose a port-Hamiltonian description of the multi-robot system to exploit universal physical constraints in interconnected systems and achieve closed-loop stability. We represent a multi-robot control policy using an architecture that combines self-attention mechanisms and neural ordinary differential equations. The former handles time-varying communication in the robot team, while the latter respects the continuous-time robot dynamics. Our representation is distributed by construction, enabling the learned control policies to be deployed in robot teams of different sizes. We demonstrate that LEMURS can learn interactions and cooperative behaviors from demonstrations of multi-agent navigation and flocking tasks.

==> 01_Intro.tex <==

%joint multi-robot 
Multi-robot systems promise improved efficiency and reliability compared to a single robot in many applications, including exploration and mapping \cite{atanasov2015decentralized,tian2022kimera}, agriculture and herding \cite{kan2021task,pierson2015bio,sebastian2021multi,sebastian2022adaptive}, and search and rescue \cite{williams2021search}. However, designing multi-robot control policies that achieve cooperative behaviors may be challenging. First, domain expertise may be required to specify the objective and constraints for a desired task in mathematical terms. Second, scaling the control policy to large teams may be computationally infeasible due to the increase of the joint state and control spaces. The first challenge motivates the use of machine learning techniques to learn reward functions or control policies from demonstration \cite{jiahao2021learning, bloembergen2015evolutionary, khan2020graph, tolstaya2020learning,tolstaya2021multi, yang2021communication, gama2022synthesizing, furieri2021distributed, han2020cooperative, shi2020neural, long2018towards, semnani2020multi, dasari2020robonet, bogert2018multi, zhu2021learning, zhou2019clone}. The second challenge motivates imposing a sparse structure in the control policy that respects the communication topology of the robot team and allows the complexity to scale with the number of neighbors rather than the total number of robots \cite{khan2020graph, tolstaya2020learning, tolstaya2021multi,yang2021communication, gama2022synthesizing, furieri2021distributed, qu2020scalable, yang2018mean, wang2022darl1n}. In this work, we develop \textbf{LEMURS} (\textbf{LE}arning distributed \textbf{MU}lti-\textbf{R}obot interaction\textbf{S}), a learning approach for distributed control synthesis from cooperative task demonstrations that generalizes to different tasks, scales favorably with the number of robots, and handles time-varying robot communication.


%With the advent of multi-robot systems, the scope of robotics has been broadened towards tasks that are impractical for a single robot system, such as cooperative exploration and mapping~\cite{atanasov2015decentralized,tian2022kimera},  agriculture or herding~\cite{kan2021task,pierson2015bio,sebastian2021multi}. However, finding a distributed optimal control policy that achieves such cooperative/competitive behaviors is challenging. First, it requires domain expertise to carefully derive the goal, costs and constraints for a particular task. Second, it is hard to scale since the problem becomes increasingly complex as the number of robots grows. This motivates the use of machine learning techniques to learn a distributed control policy from demonstration \cite{jiahao2021learning, bloembergen2015evolutionary, khan2020graph, tolstaya2020learning,tolstaya2021multi,gama2022synthesizing, han2020cooperative, furieri2021distributed, galimberti2021hamiltonian, shi2020neural}. In this paper, we develop a framework to learn distributed control policies from demonstrations that is general for different tasks, scalable with the number of robots, and compatible with time-varying communication topologies. 


%To infer the control policy, our framework models robot interactions by energy exchange among them and learn the exchange policy 

% when the task goes beyond regulation/navigation, for it is hard to define the constraints that characterize the task beyond the configurations that fulfills it. Thus, we pose the problem from a different perspective: given demonstrations, we propose a method to directly learn the multi-robot control policy that replicates an unknown task, where with unknown we meant the constraints that determines the task.

% With the advent of multi-robot systems, the scope of robotics has been broadened towards tasks that are impractical for a single robot system, such as cooperative exploration and mapping~\cite{atanasov2015decentralized,tian2022kimera},  agriculture or herding~\cite{kan2021task,pierson2015bio,sebastian2021multi}. However, finding a control policy that achieves such cooperative/competitive behaviors is challenging when the task goes beyond regulation/navigation, for it is hard to define the constraints that characterize the task beyond the configurations that fulfills it. Thus, we pose the problem from a different perspective: \textbf{given demonstrations}, we propose a method to \textbf{directly learn the multi-robot control policy} that replicates an \textbf{unknown task}, where with \textbf{unknown we meant the constraints that determines the task}.

% Machine learning techniques has recently achieved remarkable performance in learning behaviors and control of multi-robot systems. For example, neural networks have been used to model distributed control policy, whose parameters are updated using policy gradient in a reinforcement learning setting \cite{lowe2017multi, foerster2018counterfactual, zhang2021multi, bloembergen2015evolutionary}. However, this approach does not provide stability guarantees and is often hard to scale with a large number of robots.

% \NA{Separate the review of learning-based techniques for forward/inverse control from those for distributed control.}

% learning policies for inverse control 
Recent works focus on learning control policies for optimal control or reinforcement learning problems \cite{bloembergen2015evolutionary,long2018towards, semnani2020multi}. Given a cost function, a recurrent neural network \cite{zhu2021learning}, or graph convolutions and multi-layer perceptrons~\cite{zhou2019clone} have been used to learn centralized control policies. Without a cost function, inverse reinforcement learning \cite{ng2000algorithms} may be used to learn centralized \cite{dasari2020robonet,bogert2018multi} or distributed \cite{han2020cooperative} policies from task demonstrations. While black-box neural networks are widely used for learning control policies, they do not encode energy conservation and kinematic constraints satisfied by physical robot systems, and failing to infer them from data may result in unstable behaviors. A key contribution of our work is to represent the robot team as a \emph{port-Hamiltonian system} \cite{van2014port} and learn a distributed control policy from demonstration by modeling robot interactions as energy exchanges. The use of Hamiltonian mechanics has been explored for centralized control policies or fixed-time known topologies~\cite{furieri2021distributed, galimberti2021hamiltonian}, in which scalability is achieved in the absence of communication \cite{shi2020neural}. Meanwhile, our work achieves scalability with a time-varying topology by modeling robot interactions using \emph{self-attention techniques}~\cite{vaswani2017attention}.

%The Hamiltonian structure also allows us to derive a distributed control policy with stability analysis.


% \NA{Discuss why this is good}. Related work that consider Hamiltonian formulations in control policy learning includes... \NA{Methin this stuff here: ``The use of port- Hamiltonian mechanics has been explored for centralized control policies or fixed-time known communication topologies~\cite{furieri2021distributed, galimberti2021hamiltonian}, in which scalability is achieved only in the absence of communications~\cite{shi2020neural}.'' and transition to scalability with increasing number of agents.}

% distributed control
Learning and execution of control policies for multi-robot systems should scale favorably with an increasing numbers of robots. Learning a joint value or policy function is challenging due to the exponential growth of the state and action space with the size of the robot team \cite{qu2020scalable}. Successful methods for multi-agent reinforcement learning factorize value functions using a mean-field state for the team \cite{yang2018mean}, according to the $k$-hop neighborhoods \cite{wang2022darl1n,qu2020scalable} or using attention mechanisms \cite{long2020evolutionary}. Graph neural networks have been utilized as a scalable and communication-aware policy representation in coverage, exploration, and flocking problems \cite{khan2020graph, tolstaya2020learning,tolstaya2021multi,yang2021communication, gama2022synthesizing}. Recently, Li et al.~\cite{li2021message} combine graph-neural networks with self-attention to solve decentralized multi-robot path planning problems. Many of these techniques assume discrete robot dynamics, fixed or known communication topology, or prior knowledge about the task. In contrast, our approach learns a distributed control policy from demonstrated robot trajectories with an unknown task objective and handles time-varying communication and team sizes. We integrate self-attention networks with \emph{neural ordinary differential equation (ODE) networks} \cite{chen2018neural, jiahao2021learning, furieri2021distributed} to handle continuous-time dynamics even when the demonstrations are discrete. Closely related to our work, Jiahao et al. \cite{jiahao2021learning} develop a neural ODE network that learns distributed controllers but enforces collision avoidance using an explicit potential field and assumes a fixed number of neighbors. By using a port-Hamiltonian formulation and self-attention mechanism, we handle time-varying neighbors and learn constraints such as collision avoidance from data.

%Besides, the Hamiltonian structure allows us to constraint the class of learned energy-based policies such that, regardless of the setup of the task, the resulting robot trajectories do not diverge. 



% Compared to jiahao2021learning:
% fixed number of neightbors vs time varying
% Hamiltonian structure vs Potential field structure
% unstructured neural network vs IDA-PBC structure for control policy

%\TODO{Jiahao et al.~\ref{jiahao2021learning}, which develops ...}\NA{This work is quite similar to ours. It should be discussed in more detail and the differences should be highlighted. It also uses neural ODE nets.} 


% \TODO{Instead, \emph{we consider a general port- Hamiltonian formulation} of the robot dynamics~\cite{shaft2004port} and derive a class of distributed control policies that are learned from demonstration. Specifically, we model robot interactions by a \emph{novel self-attention-based  network}~\cite{vaswani2017attention,shaw2018self} that handles time-varying topology and scales with the number of robots. Our self-attention based architecture is integrated with \emph{neural ordinary differential equations networks}~\cite{chen2018neural, jiahao2021learning, furieri2021distributed}, which considers the robot continuous-time dynamics even when the demonstrations are discrete. Besides, the combination of the port-Hamiltonian formulation and the novel self-attention-based network allows us to constraint the class of learned policies to those that guarantee that, regardless of the setup of the task, the resulting robot trajectories do not diverge.}\NA{Merge our contributions into the two paragraphs above, where we discuss our method.}



% Many works learn control policies that solve an optimal control problem, with the goal, costs and constraints defined a priori. Swarm robotics~\cite{jiahao2021learning} is a typical benchmark, where neural networks and neural ordinary differential equations show successful results. Nevertheless, they are not yet generalizable to other domains; meanwhile, we seek a general solution that can be applied to a broader scope of multi-robot tasks. In this sense, reinforcement learning achieves accurate imitations of complex tasks~\cite{bloembergen2015evolutionary,long2018towards, semnani2020multi}, but the learned control policies barely scale further than a ten of robots. 
% %\textbf{Scalability is a limitation that our proposal aims to address}. 
% Graph neural networks are an alternative to obtain scalable and communication-aware solutions. They have been explored to learn distributed controllers~\cite{khan2020graph} for coverage, exploration or flocking~\cite{tolstaya2020learning,tolstaya2021multi,gama2022synthesizing}. However, they still need prior knowledge about the task, e.g., a fixed communication topology. 
% Instead, we aim to learn control policies for time-varying numbers of robots and topologies. 
% %On the contrary, \textbf{we aim to achieve distributed and stable control policies directly from demonstrations}.

% Some recent works address the problem of learning control policies when the task constraints, costs or goals are unknown. Inverse reinforcement learning~\cite{ng2000algorithms} extracts the reward function that characterizes the task, which is then used to learn centralized~\cite{dasari2020robonet,bogert2018multi} or distributed~\cite{han2020cooperative} navigation and collision avoidance policies.  %With the same purpose, Zhu et al.~\cite{zhu2021learning} propose a 
% A recurrent neural network and a model predictive control policy~\cite{zhu2021learning}, or graph convolutions and multi-layer perceptrons~\cite{zhou2019clone} have been used to learn centralized control policies. However, these works assume discrete-time robot dynamics and do not encode universal continuous-time physics laws of robot systems, such as Lagrangian or Hamiltonian mechanics in the control design. As a result, the control policy model might struggle to infer these laws from data. The use of port- Hamiltonian mechanics has been explored for centralized control policies or fixed-time known communication topologies~\cite{furieri2021distributed, galimberti2021hamiltonian}, in which scalability is achieved only in the absence of communications~\cite{shi2020neural}. 
% %that is learned from demonstrations, while Zhou et al.~\cite{zhou2019clone} use graph convolutions and multi-layer perceptrons to learn a centralized swarm policy. 
% %These solutions are not general, distributed nor guarantee stability. 
% Instead, \emph{we consider a general port- Hamiltonian formulation} of the robot dynamics~\cite{shaft2004port} and derive a class of distributed control policies that are learned from demonstration. Specifically, we model robot interactions by a \emph{novel self-attention-based  network}~\cite{vaswani2017attention,shaw2018self} that handles time-varying topology and scales with the number of robots. Our self-attention based architecture is integrated with \emph{neural ordinary differential equations networks}~\cite{chen2018neural, jiahao2021learning, furieri2021distributed}, which considers the robot continuous-time dynamics even when the demonstrations are discrete. Besides, the combination of the port-Hamiltonian formulation and the novel self-attention-based network allows us to constraint the class of learned policies to those that guarantee that, regardless of the setup of the task, the resulting robot trajectories do not diverge. 

%Self-attention networks remain to be explored beyond multi-robot path planning~\cite{he2021deepcc,kamra2020multi,li2021message}

In summary, we develop LEMURS, a novel algorithm for learning scalable multi-robot control policies from demonstration. Our \emph{first contribution} is the use of port-Hamiltonian dynamics to restrict the family of learned policies to those that are stable and distributed. Our \emph{second contribution} is a novel learning architecture that integrates concepts of self-attention and neural ODEs to handle continuous-time dynamics, time-varying communication, and large robot teams. 

% Therefore, we can learn the control policy with only a few robots and accurately deploy it in much larger teams.
% (\textbf{LE}arning distributed \textbf{MU}lti-\textbf{R}obot interaction\textbf{S})

==> 02_ProblemStatement.tex <==
Consider a team of robots, indexed by $\mathcal{V} = \{1, \hdots, n \}$. Assume that the dynamics of each robot $i \in \mathcal{V}$ are \emph{known}:
%
\begin{equation}\label{eq:known_dynamics}
    \dot{\mathbf{x}}_i(t) = \bff_i(\mathbf{x}_i(t),\mathbf{u}_i(t)),
\end{equation}
%
%\footnote{\textbf{Notation}: We use lower-case letters for scalars and functions, bold lower-case letters for vectors, bold capital letters for matrices, and calligraphic capital letters for sets. We use the symbol $\geq$ for greater than or equal, $\succeq$ for positive semidefinite, ${\;}^\top$ for transpose, $\dot{\;}$ for time-derivative, ${\;}^{\dagger}$ for right pseudoinverse, $\mathsf{sign}(\;)$ for the sign function, $\mathsf{diag}(\;)$ for the diagonal of a matrix, and $||{\;}||_{p}$ for the $p$-norm of a vector/matrix. We use $[{\;}]_{ij}$ to denote the $ij$-th element or block of a matrix and $|\;|$ for the cardinality of a set.
%, and $\mathsf{Re}(\;)$ for the real part of a complex number. We denote the $p \times p$ identity matrix by $\mathbf{I}_p$, the zero matrix of appropriate dimension by $\mathbf{0}$, and a column vector of ones by $\mathbf{1}$. }\TD{To save space, do we need this footnote as most of these notations are standard or can be defined when they are first mentioned?}
where $\mathbf{x}_i(t) \in \mathbb{R}^{n_x}$ and $\mathbf{u}_i(t) \in \mathbb{R}^{n_u}$ denote the state and control input of the robot at time $t\geq0$. The robots interact in a distributed manner, described by a time-varying undirected graph $\mathcal{G}(t) = (\mathcal{V},\mathcal{E}(t))$, where $\mathcal{E}(t) \subseteq \mathcal{V} \times \mathcal{V}$ is the set of edges. An edge $(i,j) \in \mathcal{E}(t)$ exists when robots $i$ and $j$ interact at time $t$. Robot $i$ can always interact with itself, i.e., $(i,i) \in \calE(t)$ for all $i$, $t$. Let $\mathbf{A}(t) \in \{0,1\}^{n \times n}$ be the weighted adjacency matrix associated to $\mathcal{G}(t)$, such that $[\mathbf{A}(t)]_{ij} \neq 0$ if and only if $(i,j) \in \mathcal{E}(t)$, and $0$ otherwise. The set of $k$-hop neighbors of robot $i$ at $t$ is $\mathcal{N}_i^k(t) = \{j \in \mathcal{V} \mid [\mathbf{A}^k(t)]_{ij} \neq 0 \}$. 
%Let $\mathbf{A}(t)$ be the adjacency matrix associated with $\mathcal{G}(t)$ such that $[\mathbf{A}(t)]_{ij} = 1$, if $(i,j) \in \mathcal{E}(t)$, and $[\mathbf{A}(t)]_{ij} = 0$, otherwise. The diagonal degree matrix $\mathbf{D}(t)$ of $\mathcal{G}(t)$ contains the number of neighbors of each node on its diagonal, i.e., $\mathsf{diag}(\mathbf{D}(t)) = \mathbf{A}(t) \mathbf{1}$ and $[\mathbf{D}(t)]_{ij} = 0$, $\forall i \neq j$. Finally, the Laplacian matrix of $\mathcal{G}(t)$ is $\mathbf{L}(t) = \mathbf{D}(t) - \mathbf{A}(t)$. We denote by $\mathsf{wspace}(\mathbf{L})$ the space of weighted matrices that have the same dimension as $\mathbf{L}$ and satisfy $[\mathbf{L}^{\prime}]_{ij} \neq 0$ if $[\mathbf{L}]_{ij} \neq 0$, $\mathsf{sign}([\mathbf{L}^{\prime}]_{ij}) =  \mathsf{sign}([\mathbf{L}]_{ij})$ and $(\mathbf{L}^{\prime} - \mathbf{I}\mathsf{diag}(\mathbf{L}^{\prime}))\mathbf{1} = \mathbf{0}$.
Each robots executes an \emph{unknown} control policy:
% \begin{equation}\label{eq:general_controller}
%     \mathbf{u}_i(t) = \pi \left(\mathbf{x}_i(t), \{\mathbf{x}_j(t)\}_{j\in{\mathcal{N}_i(t)}}, \bm{\theta}\right),
% \end{equation}
\begin{equation}\label{eq:general_controller}
    \mathbf{u}_i(t) = \bfpi_{\bftheta}\left(\bfx_{\calN_i^k}(t)\right),
\end{equation}
where $\bfx_{\calN_i^k}(t) = \{\bfx_j(t) \mid j \in \calN_i^k(t)\}$ and $\bftheta$ is the control policy parameters. Our objective is to use task demonstrations to learn $\bftheta$, such that the multi-robot team, following the learned control policy, replicates the task. 

\begin{example}\label{example:flocking_controller}
To illustrate the problem setting, consider a flocking task \cite{olfati2006flocking} in which a robot team must achieve a formation with aligned velocities, while avoiding collisions. The robots follow double integrator dynamics $\dot{\mathbf{p}}_i(t) = \mathbf{v}_i(t)$ and $\dot{\mathbf{v}}_i(t) = \mathbf{u}_i(t)$, where $\mathbf{p}_i(t) \in \mathbb{R}^m$, $\mathbf{v}_i(t) \in \mathbb{R}^m$, and $\mathbf{u}_i(t) \in \mathbb{R}^m$ are the position, velocity, and input of robot~$i$. A distributed control policy that achieves flocking was developed by Olfati-Saber \cite{olfati2006flocking}:
%
\begin{align}
    \mathbf{u}_i(t) =& - c_1\mathbf{p}_i(t) - c_2\mathbf{v}_i(t) + \kern -0.3cm \sum_{j \in \mathcal{N}^1_i(t)} \kern -0.3cm \phi(||\Delta\mathbf{p}_{ij}(t)||_{\sigma})\mathbf{n}_{ij}(t) 
    \notag\\&
    + \kern -0.2cm \sum_{j \in \mathcal{N}^1_i(t)}\kern -0.2cm \rho\left(||\Delta\mathbf{p}_{ij}(t)||_{\sigma}\right)(\mathbf{v}_{j}(t)-\mathbf{v}_i(t))
    % \notag\\&
     \label{eq:real_flocking_controller}
\end{align}
where $\Vert{\cdot}\Vert_{\sigma}$ denotes the $\sigma$-norm of a vector and $\Delta\mathbf{p}_{ij}(t) = \mathbf{p}_{j}(t)-\mathbf{p}_i(t)$.
%
The first and second terms are a proportional controller with gains $c_1,c_2>0$ that prevents the formation of sub-flocks, where we have assumed $\mathbf{p}_i(t) = \mathbf{v}_i(t) = \mathbf{0}$ $\forall i$ as the desired flock configuration. The third term avoids robot collisions and induces the desired lattice formation, where $\phi(\cdot)$ is a potential function whose minima are located at the desired inter-robot distances, and $\mathbf{n}_{ij}(t)$ is a vector that points in the repulsion/coalition direction.  The last term achieves velocity consensus using a distance scaling function $\rho(\cdot)$ that models the robot communication. Further details can be found in \cite{olfati2006flocking}. This paper aims to learn policies like \eqref{eq:real_flocking_controller} from demonstrations.
\end{example}




%We define the joint state and control input as $$\mathbf{x} := [\mathbf{x}_1^\top, \hdots, \mathbf{x}_n^\top]^\top, \quad \mathbf{u} := [\mathbf{u}_1^\top, \hdots, \mathbf{u}_n^\top]^\top.$$

%We assume that we are able to collect state-trajectories from demonstrations of other agents, e.g., trajectories of an actual flock, leading to successful interactions and task executions. 
% The collection of multiple trajectories builds the dataset $\bar{\mathcal{D}} := \{ \bar{\mathbf{x}}_{0:K}^l \}_{l=0}^{l=L}$, with $L>0$ the number of trajectories. The corresponding generated trajectories is $\mathcal{D} := \{ \mathbf{x}_{0:K}^l \}_{l=0}^{l=L}$. 


We assume that state trajectories from successful task executions are available as training data. Let $\mathbf{x}(t) = [\mathbf{x}_1^\top(t), \ldots, \mathbf{x}_n^\top(t)]^\top$ and $\mathbf{u}(t) = [\mathbf{u}_1^\top(t), \ldots, \mathbf{u}_n^\top(t)]^\top$ denote the joint state and control of the robot team. Given an initial state $\mathbf{x}(0) = \mathbf{x}_0$, let $\bar{\mathbf{x}}_{0:K} := [\bar{\mathbf{x}}(0), \hdots, \bar{\mathbf{x}}(rT), \hdots, \bar{\mathbf{x}}(KT)]$ and $\mathbf{x}_{0:K} := [\mathbf{x}(0), \hdots, \mathbf{x}(rT), \hdots, \mathbf{x}(KT)]$ be demonstrated and learned policy's trajectories, respectively, with $K$ denoting the number of discrete samples $r$ along the trajectories with sampling interval $T$. Let $\bar{\mathcal{D}} := \{ \bar{\mathbf{x}}_{0:K}^l \}_{l=0}^{l=L}$ denote a dataset of $L >0$ demonstrated trajectories. Let $\mathcal{D} := \{ \mathbf{x}_{0:K}^l \}_{l=0}^{l=L}$ be the generated trajectories under policy $\pi_{\bftheta}$. We aim to learn a control policy that minimizes the distance between the demonstrated and generated trajectories:
%
\begin{equation}\label{eq:loss_function}
    \mathcal{L}({\mathcal{D}},\bar{\mathcal{D}}) = \frac{1}{KL}\sum_{l=0}^L\sum_{r=0}^K
    ||\mathbf{x}^l(rT)-\bar{\mathbf{x}}^l(rT)||^2_2.
\end{equation}
%
Formally, the problem we consider is:
%
\begin{subequations}\label{eq:prob_def}
\begin{alignat}{2}
\min_{\bftheta} & \hbox{ }       \mathcal{L}({\mathcal{D}},\bar{\mathcal{D}}) \label{eq:prob_def_cost}
\\
\text{s.t.} & \hbox{ }\dot{\mathbf{x}}_{i}^l(t) = \bff_i(\mathbf{x}_i^l(t), \mathbf{u}_i^l(t)), \hbox{ } \bfx_i^l(0) = \bar{\bfx}_i^l(0), \hbox{ } \forall i,l,\label{eq:prob_def_constraint2}
\\
& \hbox{ } {\mathbf{u}}_i^l(t) = \bfpi_{\bftheta}(\bfx^l_{\calN_i^{k}}(t)), \hbox{ } \forall i,l,t. \label{eq:prob_def_constraint3}
\end{alignat}
\end{subequations}
%
As specified in the formulation above, the learned control policy should also handle time-varying communication and should be adaptable to changes in the total number of robots or the number of neighbors for each robot.


%Moreover, we also seek a control policy that uses only local and neighboring information, is implementable in teams of any number of robots and time-varying communication topologies, and avoids the divergence of robots trajectories when they are deployed in a new task setup.

%In the next section we describe the proposed solution for problem~\eqref{eq:prob_def}.

% By combining Eqs.~\eqref{eq:simple} and~\eqref{eq:general_controller}, the overall closed-loop dynamics of the multi-robot system is
% % \NA{It is best to avoid using abbreviations unless it is our own method LEMURS.}\ES{Done.} 
% \begin{equation}\label{eq:closed_loop}
%     \dot{\mathbf{x}}(t)=f(\mathbf{x}(t)).   
% \end{equation}
% Our purpose is to identify $f(\cdot)$ by means of $\pi(\cdot)$. In other words, we aim at identifying the controller that captures the closed-loop dynamics in Eq.~\eqref{eq:closed_loop}. 




==> 03_ProposedSolution.tex <==


In this section, we present a port-Hamiltonian formulation of the multi-robot dynamics and an energy-based distributed control design that can shape the interactions and Hamiltonian of the closed-loop system (Sec.~\ref{subsec:portHamiltonian}). Given task demonstrations, we employ self-attention and neural ordinary differential equations to learn the interactions and energy parameters of the control policy that minimize the distance between the demonstrated and generated trajectories (Sec. \ref{subsec:LEMURS}). To simplify the notation, we omit the time dependence of the states $\bfx$ and controls $\bfu$ in the reminder of the paper.

%Given demonstrated state trajectories of a task, the Hamiltonian structure allows us to learn robot interactions and a distributed, scalable control policy from demonstration that avoids potential robots divergences, using self-attention techniques and neural ordinary differential equation networks (Sec. \ref{subsec:LEMURS}). In the following, we omit the time-dependency in $\mathbf{x}$ and $\mathbf{u}$ for readability. 

%In this Section the technical approach to solve problem~\eqref{eq:prob_def} is presented. In Subsection~\ref{subsec:portHamiltonian} we move from the individual robot to the system dynamics by means of port-Hamiltonian mechanics, showing the convenience of this formulation in terms of stability, scalability and distributed behavior. In Subsection~\ref{subsec:LEMURS} we return to the robot dynamics level to present the learning proposal to solve~\eqref{eq:prob_def}.  

\subsection{Port-Hamiltonian Formulation of Multi-Robot Dynamics}\label{subsec:portHamiltonian}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% As a physical system, the individual robot dynamics \eqref{eq:known_dynamics} formulated in Section~\ref{sec:prosta} satisfy port- Hamiltonian mechanics \cite{van2014port, lee2017global, duong2021hamiltonian} for $i = 1, \ldots, n$:
% , lee2017global, duong2021hamiltonian

Since robots are physical systems that satisfy Hamiltonian mechanics, we model each robot's dynamics in \eqref{eq:known_dynamics} as a port-Hamiltonian system \cite{van2014port}:
%
\begin{equation}\label{eq:open_loop_intro_individual}
        \dot{\mathbf{x}}_i = \left(\mathbf{J}_s^{(i)}(\mathbf{x}_i) - \mathbf{R}_s^{(i)}(\mathbf{x}_i)\right) \frac{\partial {H}_s^{(i)}(\mathbf{x}_i)}{\partial\mathbf{x}_i}
        + \mathbf{F}_s^{(i)}(\mathbf{x}_i)\mathbf{u}_i,
\end{equation}
%
where the skew-symmetric interconnection matrix $\mathbf{J}_s^{(i)}(\bfx_i)$ represents energy exchange \emph{within a robot}, the positive-semidefinite dissipation matrix $\bfR_s^{(i)}(\bfx_i)$ represents energy dissipation, the Hamiltonian ${H}_s^{(i)}(\mathbf{x}_i)$ represents the total energy, and the matrix $\bfF_s^{(i)}(\bfx_i)$ is the input gain.

% , consisting of $n$ robots,
Then, the multi-robot system with joint state $\bfx$ also follows port-Hamiltonian dynamics:
%
\begin{equation}\label{eq:open_loop_intro}
        \dot{\mathbf{x}} =  \left(\mathbf{J}_s(\mathbf{x})  -  \mathbf{R}_s(\mathbf{x})\right)\frac{\partial {H}_s(\mathbf{x})}{\partial\mathbf{x}}  +  \mathbf{F}_s(\mathbf{x})\mathbf{u},
\end{equation}
%
where $\mathbf{J}_s(\bfx)$, $\bfR_s(\bfx)$, and $\bfF_s^{(i)}(\bfx)$ are block-diagonal:
%
\begin{equation}\label{eq:block_diag_structure}
\begin{aligned}
    \bfJ_s(\bfx) &= \text{diag}\left(\bfJ_s^{(1)}(\bfx_1), \ldots, \bfJ_s^{(n)}(\bfx_n) \right), \\
    \bfR_s(\bfx) &= \text{diag}\left(\bfR_s^{(1)}(\bfx_1), \ldots, \bfR_s^{(n)}(\bfx_n) \right), \\
    \bfF_s(\bfx) &= \text{diag}\left(\bfF_s^{(1)}(\bfx_1), \ldots, \bfF_s^{(n)}(\bfx_n) \right), \\
\end{aligned}
\end{equation}
%
and $H_s(\bfx) = \sum_{i=1}^n H_s^{(i)}(\bfx_i)$.

Without control, the trajectories of the open-loop system in \eqref{eq:open_loop_intro} would not match the demonstrations in $\bar{\calD}$. The dynamics need to be controlled by the policy in \eqref{eq:general_controller} in order to generate desired trajectories. We employ an interconnection and damping assignment passivity-based control (IDA-PBC) approach \cite{van2014port}, which injects additional energy to the system through the control input $\bfu$ to achieve some closed-loop dynamics that replicate the demonstrated task:
%
\begin{equation}\label{eq:closed_loop_intro}
        \dot{\mathbf{x}} = \left( \mathbf{J}_{\bftheta}(\mathbf{x})   -   \mathbf{R}_{\bftheta}(\mathbf{x})\right)
\frac{\partial {H_{\bftheta}}(\mathbf{x})}{\partial\mathbf{x}}, 
\end{equation}
%
with Hamiltonian $H_{\bftheta}(\bfx)$, skew-symmetric interconnection $\mathbf{J}_{\bftheta}(\mathbf{x})$, and positive semidefinite dissipation $\mathbf{R}_{\bftheta}(\mathbf{x})$. By matching the terms in \eqref{eq:open_loop_intro} and \eqref{eq:closed_loop_intro}, one obtains the policy:
%
\begin{equation}\label{eq:open_loop_intro_controller}
\begin{aligned}
\mathbf{u} &= \mathbf{F}_s^{\dagger}(\mathbf{x})
\left( \left(\mathbf{J}_{\bftheta}(\mathbf{x}) - \mathbf{R}_{\bftheta}(\mathbf{x})\right)\frac{\partial {H_{\bftheta}}(\mathbf{x})}{\partial\mathbf{x}} \right. 
\\
& \qquad \quad \kern 0.2cm- \left.\left(\mathbf{J}_s(\mathbf{x}) - \mathbf{R}_s(\mathbf{x})\right)\frac{\partial {H}_s(\mathbf{x})}{\partial\mathbf{x}} \right),
\end{aligned}
\end{equation}
%
where $\mathbf{F}_s^{\dagger}(\mathbf{x}) = \left(\bfF_s^{\top}(\bfx)\bfF_s(\bfx)\right)^{-1}\bfF_s^{\top}(\bfx)$ is the pseudo-inverse of $\mathbf{F}_s(\mathbf{x})$. 
% The control $\bfu$ in \eqref{eq:open_loop_intro_controller} achieves the desired closed-loop dynamics as long as the following matching condition is satisfied:
% %
% \begin{equation}\label{eq:matching_condition}
% \begin{aligned}
% \mathbf{F}_s^{\perp}(\mathbf{x})
% & \left( \left(\mathbf{J}_{\bftheta}(\mathbf{x}) - \mathbf{R}_{\bftheta}(\mathbf{x})\right)\frac{\partial {H_{\bftheta}}(\mathbf{x})}{\partial\mathbf{x}} \right.
% \\
% &-
% \left.\left(\mathbf{J}_s(\mathbf{x}) - \mathbf{R}_s(\mathbf{x})\right)\frac{\partial {H}_s(\mathbf{x})}{\partial\mathbf{x}} \right) = 0,
% \end{aligned}
% \end{equation}
% %
% where $\mathbf{F}_s^{\perp}(\mathbf{x})$ is the maximal-rank left annihilator of $\mathbf{F}_s(\mathbf{x})$, i.e. $\mathbf{F}_s^{\perp}(\mathbf{x})\mathbf{F}_s(\mathbf{x}) = 0$. 
If the robots are fully-actuated, i.e., $\bfF_s(\bfx)$ is full-rank, the matching condition on the pseudo-inverse is always satisfied, achieving the desired closed-loop dynamics. For underactuated systems, satisfaction of the matching condition may not always be possible \cite{blankenstein2002matching}. Being able to achieve zero error $\calL(\calD,\bar{\calD})$ is, hence, related to whether the demonstrated trajectories $\bar{\calD}$ are realizable by the class of control policies in \eqref{eq:open_loop_intro_controller}. Even if the trajectories in $\bar{\calD}$ are not realizable, the policy parameters $\bftheta$ may still be optimized to achieve a behavior as similar as possible.

Let $[\mathbf{J}_{\bftheta}(\mathbf{x})]_{ij}$ and $[\mathbf{R}_{\bftheta}(\mathbf{x})]_{ij}$ denote the $n_x \times n_x$ blocks with index $(i,j)$, representing the energy exchange between robot $i$ and $j$ and the energy dissipation of robot $i$ caused by robot $j$, respectively. Since the input gain $\mathbf{F}_s(\mathbf{x})$ in \eqref{eq:block_diag_structure} is block-diagonal, the individual control policy of robot $i$ is:
%
\begin{equation}\label{eq:open_loop_intro_controller_ind}
\begin{aligned}
\kern -5pt \mathbf{u}_i &= \mathbf{F}_s^{(i)\dagger}(\mathbf{x}_i)
\left( \sum_{j \in \calV}\left([\mathbf{J}_{\bftheta}(\mathbf{x})]_{ij} - [\mathbf{R}_{\bftheta}(\mathbf{x})]_{ij}\right)\frac{\partial H_{\bftheta}(\mathbf{x})}{\partial \mathbf{x}_j}\right. 
\\
& \qquad \quad \kern 0.3cm- \left.\left(\mathbf{J}_s^{(i)}(\mathbf{x}_i) - \mathbf{R}_s^{(i)}(\mathbf{x}_i)\right)\frac{\partial {H}_s^{(i)}(\mathbf{x})}{\partial\mathbf{x}_i} \right).
\end{aligned}
\end{equation}
%
The individual control policies in \eqref{eq:open_loop_intro_controller_ind} do not necessarily respect the hops in the communication network as desired in \eqref{eq:general_controller} because this depends on the structure of $\mathbf{J}_{\bftheta}(\mathbf{x})$,  $\mathbf{R}_{\bftheta}(\mathbf{x})$, and $H_{\bftheta}(\bfx)$. In Sec.~\ref{subsec:LEMURS}, we impose conditions on these terms to ensure that they respect the communication topology and are skew-symmetric, and positive semidefinite, respectively, as required for a valid port-Hamiltonian system.



%In Sec. \ref{subsec:LEMURS}, we derive the the requirements for the controller \eqref{eq:open_loop_intro_controller_ind} and design our model of robot interactions and control policy, inheriting stability guarantees from the IDA-PBC approach while staying distributed.


% As the control input $\bfu_i$ only affects the robot $i$, the input gain matrix $\mathbf{F}_s(\mathbf{x})$ is block-diagonal: 
% \begin{equation}
%     \bfF_s(\bfx) = \text{diag}\prl
% {\bfF_s^{(1)}(\bfx_1), \ldots, \bfF_s^{(n)}(\bfx_n)},
% \end{equation}
% where $\bfF_s^{(i)}(\bfx_i)$ is the input gain matrix for robot $i$. This allows each robot $i$ to evaluate the matching conditions and calculate its control input $\bfu_i$ locally using \eqref{eq:open_loop_intro_controller}. 



% Given a desired state $\bfx^*$, the original Hamiltonian system \eqref{eq:open_loop_intro} without any control input does not converge to $\bfx^*$ as the total energy $H_s(\bfx)$ is not minimized at $\bfx^*$. To drive the system to $\bfx^*$, we employ the interconnection
% and damping assignment passivity-based control (IDA-PBC) approach \cite{van2014port}, which injects additional energy to the system through the control input $\bfu$ so that the system has a desired total energy $H(\bfx)$ with a minimizer $\bfx^*$. The closed-loop multi-robot system, i.e., with a control policy $\bfu = \bfpi(\bfx)$, satisfies a desired Hamiltonian dynamics:
% \begin{equation}\label{eq:closed_loop_intro}
%         \dot{\mathbf{x}} = \left( \mathbf{J}(\mathbf{x})   -   \mathbf{R}(\mathbf{x})\right)
% \frac{\partial {H}(\mathbf{x})}{\partial\mathbf{x}}, 
% \end{equation}
% where $\bfJ(\bfx)$ and $\bfR(\bfx)$ are the desired skew-symmetric interconnection and positive semidefinite dissipation matrices. Eq.~\eqref{eq:closed_loop_intro} represents the task to replicate. 
% By matching \eqref{eq:open_loop_intro} and \eqref{eq:closed_loop_intro}, the control input is as follows:
% \begin{equation}\label{eq:open_loop_intro_controller}
% \begin{aligned}
% \mathbf{u} &= \mathbf{F}_s^{\dagger}(\mathbf{x})
% \left( \left(\mathbf{J}(\mathbf{x}) - \mathbf{R}(\mathbf{x})\right)\frac{\partial {H}(\mathbf{x})}{\partial\mathbf{x}} \right. 
% \\
% & \qquad \quad \kern 0.2cm- \left.\left(\mathbf{J}_s(\mathbf{x}) - \mathbf{R}_s(\mathbf{x})\right)\frac{\partial {H}_s(\mathbf{x})}{\partial\mathbf{x}} \right),
% \end{aligned}
% \end{equation}
% where $\mathbf{F}_s^{\dagger}(\mathbf{x}) = \left(\bfF_s^{T}(\bfx)\bfF_s(\bfx)\right)^{-1}\bfF_s^{T}(\bfx)$ is the pseudo-inverse of $\mathbf{F}_s(\mathbf{x})$. The control $\bfu$ exists as long as the following matching conditions are satisfied:
% \begin{equation}\label{eq:matching_condition}
% \begin{aligned}
% \mathbf{F}_s^{\perp}(\mathbf{x})
% & \left( \left(\mathbf{J}(\mathbf{x}) - \mathbf{R}(\mathbf{x})\right)\frac{\partial {H}(\mathbf{x})}{\partial\mathbf{x}} \right.
% \\
% &-
% \left.\left(\mathbf{J}_s(\mathbf{x}) - \mathbf{R}_s(\mathbf{x})\right)\frac{\partial {H}_s(\mathbf{x})}{\partial\mathbf{x}} \right) = 0,
% \end{aligned}
% \end{equation}
% where $\mathbf{F}_s^{\perp}(\mathbf{x})$ is the maximal-rank left annihilator of $\mathbf{F}_s(\mathbf{x})$, i.e. $\mathbf{F}_s^{\perp}(\mathbf{x})\mathbf{F}_s(\mathbf{x}) = 0$. 
% As the control input $\bfu_i$ only affects the robot $i$, the input gain matrix $\mathbf{F}_s(\mathbf{x})$ is block-diagonal: 
% \begin{equation}
%     \bfF_s(\bfx) = \text{diag}\prl
% {\bfF_s^{(1)}(\bfx_1), \ldots, \bfF_s^{(n)}(\bfx_n)},
% \end{equation}
% where $\bfF_s^{(i)}(\bfx_i)$ is the input gain matrix for robot $i$. This allows each robot $i$ to evaluate the matching conditions and calculate its control input $\bfu_i$ locally using \eqref{eq:open_loop_intro_controller}. 

% Assuming the matching conditions are satisfied, e.g., when each robot is fully-actuated, i.e., $\bfF_s(\bfx)$ is full-rank, the closed-loop system \eqref{eq:closed_loop_intro} is stable around $\bfx^*$ in the sense of Lyapunov \cite{van2014port} with $\partial {H}(\bfx)/\partial \bfx = \mathbf{0}$ at $\bfx = \bfx^*$. In the control policy \eqref{eq:open_loop_intro_controller}, $\bfJ_s(\bfx)$, $\bfR_s(\bfx)$, $\bfF_s(\bfx)$ and $H_s(\bfx)$ are known terms from the robot individual dynamics. Meanwhile, $\bfJ(\bfx)$, $\bfR(\bfx)$, $\bfF(\bfx)$ and $H(\bfx)$ must be designed such that the closed-loop system converges to $\bfx^*$ and fulfills the task.

% %$[\mathbf{J}(\mathbf{x})]_{i}$ and $[\mathbf{R}(\mathbf{x})]_{i}$ denote the $i$th $n_x \times n n_x$ row blocks and 
% Given demonstrated state trajectories, the Hamiltonian structure and the IDA-PBC control design \eqref{eq:open_loop_intro_controller} reduce the problem of learning the control policy in \eqref{eq:prob_def} to finding a desired skew-symmetric interconnection matrix $\mathbf{J}(\mathbf{x})$, a desired positive semidefinite dissipation matrix $\mathbf{R}(\mathbf{x}) \succeq \mathbf{0}$ and a desired Hamiltonian ${H}(\mathbf{x})$ to minimize the loss function \eqref{eq:loss_function}. Let $[\mathbf{J}(\mathbf{x})]_{ij}$ and $[\mathbf{R}(\mathbf{x})]_{ij}$ denote the $n_x \times n_x$ blocks with index $(i,j)$, representing the energy exchange between robot $i$ and robot $j$ and energy dissipation of robot $i$ caused by robot $j$, respectively. Thus, the IDA-PBC controller \eqref{eq:open_loop_intro_controller} yields to the following individual control policy $\pi(\;)$:
% \begin{equation}\label{eq:open_loop_intro_controller_ind}
% \begin{aligned}
% \kern -5pt \mathbf{u}_i &= \mathbf{F}_s^{\dagger}(\mathbf{x}_i)
% \left( \sum_{j \in \calV}\left([\mathbf{J}(\mathbf{x})]_{ij} - [\mathbf{R}(\mathbf{x})]_{ij}\right)\frac{\partial H(\mathbf{x})}{\partial \mathbf{x}_j}\right. 
% \\
% & \qquad \quad \kern 0.2cm- \left.\left(\mathbf{J}_s^{(i)}(\mathbf{x}_i) - \mathbf{R}_s^{(i)}(\mathbf{x}_i)\right)\frac{\partial {H}_s^{(i)}(\mathbf{x})}{\partial\mathbf{x}_i} \right),
% \end{aligned}
% \end{equation}
% leading to the closed-loop dynamics of robot $i$
% \begin{equation}\label{eq:individual_dynamics_notdistributed}
%     \dot{\mathbf{x}}_i = \sum_{j \in \calV}([\mathbf{J}(\mathbf{x})]_{ij}-[\mathbf{R}(\mathbf{x})]_{ij})\frac{\partial H(\mathbf{x})}{\partial \mathbf{x}_j}.
% \end{equation}


% \begin{equation} \label{eq:JRH_conditions}
%     \begin{aligned}
%         \frac{\partial}{\partial \bfx_j}\prl{\frac{\partial H}{\partial \bfx_i}} &=& \mathbf{0}, \quad\forall j \notin \calN_i \\
%         [\mathbf{J}(\mathbf{x})]_{ij} & = & \mathbf{0}, \quad\forall j \notin \calN_i \\
%         [\mathbf{R}(\mathbf{x})]_{ij} & = & \mathbf{0}, \quad\forall j \notin \calN_i.
%     \end{aligned}
% \end{equation}
%In Sec. \ref{subsec:LEMURS}, we derive the the requirements for the controller \eqref{eq:open_loop_intro_controller_ind} and design our model of robot interactions and control policy, inheriting stability guarantees from the IDA-PBC approach while staying distributed.

%In other words, by using the port- Hamiltonian formulation, we transform the original problem, an unstructured learning problem within a large class of control policies, to a structured learning problem within a tighter class of stable and distributed control policies by construction. 
%In the next Subsection we propose a solution to learn $\mathbf{R}(\mathbf{x}), \mathbf{J}(\mathbf{x})$ and ${H}(\mathbf{x})$ such that they respect both the port-Hamiltonian, stability and distributed constraints.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The dynamics formulated in Section~\ref{sec:prosta} is completely unstructured, for there is no particular restriction in the class of policies that solve problem~\eqref{eq:prob_def}. This hinders the learning problem because the control policy not only has to accomplish the task, but also it must guarantee a stable and distributed behavior of the multi-robot team in order to succeed in general settings. We propose a port-Hamiltonian~\cite{shaft2004port} description of the system to exploit universal physical constraints over networked systems and guarantee a stable and distributed control policy by construction.

% The port-Hamiltonian description of a general interconnected system is 
% \begin{equation}\label{eq:closed_loop_intro}
%         \dot{\mathbf{x}} = \left( \mathbf{J}(\mathbf{x})   -   \mathbf{R}(\mathbf{x})\right)
% \frac{\partial {H}(\mathbf{x})}{\partial\mathbf{x}}, 
% \end{equation}
% where ${H}(\mathbf{x}) \geq 0$ is the \textbf{Hamiltonian} (i.e., total energy) of the system, $\mathbf{J}(\mathbf{x})$ is a skew-symmetric \textbf{interconnection matrix} ($\mathbf{J}(\mathbf{x}) + \mathbf{J}^T(\mathbf{x}) = \mathbf{0}$), and $\mathbf{R}(\mathbf{x})$ is a positive semidefinite \textbf{dissipation matrix} ($\mathbf{R}(\mathbf{x}) \succeq \mathbf{0}$). In terms of the multi-robot system,  $\mathbf{J}(\mathbf{x})$ and $\mathbf{R}(\mathbf{x})$ model how robots interact (by exchanging and dissipating energy) so that the system converges to a minimum-energy equilibrium point that corresponds to the fulfillment of the task. Nevertheless, Eq.~\eqref{eq:closed_loop_intro} is the closed-loop dynamics of the system. In the absence of a known controller, the multi-robot system is described by open-loop input-state-output port-Hamiltonian dynamics 
% \begin{equation}\label{eq:open_loop_intro}
%         \dot{\mathbf{x}} = \left(\mathbf{J}_s(\mathbf{x}) - \mathbf{R}_s(\mathbf{x})\right)\frac{\partial {H}_s(\mathbf{x})}{\partial\mathbf{x}} + \mathbf{F}_s^T(\mathbf{x})\mathbf{u}.
% \end{equation}
% Here, ${H}_s(\mathbf{x}), \mathbf{J}_s(\mathbf{x}), \mathbf{R}_s(\mathbf{x})$ are the open-loop Hamiltonian, interconnection matrix and dissipation matrix respectively, and $\mathbf{F}_s(\mathbf{x})$ is an input matrix. The aim of the control policy is to obtain Eq.~\eqref{eq:closed_loop_intro} from Eq.~\eqref{eq:open_loop_intro}. Interestingly, the port-Hamiltonian description allows to define the controller as another energy system with a port-Hamiltonian description~\cite{yuksel2014reshaping}, since the interconnection of two port-Hamiltonian systems is another port-Hamiltonian system~\cite{shaft2004port}. In particular, the interconnection
% and damping assignment passivity-based controller (IDA-PBC) 
% \begin{equation}\label{eq:open_loop_intro_controller}
% \begin{aligned}
% \mathbf{u} =& \mathbf{F}_s^{\dagger}(\mathbf{x})
% \left( \left(\mathbf{J}(\mathbf{x}) - \mathbf{R}(\mathbf{x})\right)\frac{\partial {H}(\mathbf{x})}{\partial\mathbf{x}} \right.
% \\
% & 
% -
% \left.\left(\mathbf{J}_s(\mathbf{x}) - \mathbf{R}_s(\mathbf{x})\right)\frac{\partial {H}_s(\mathbf{x})}{\partial\mathbf{x}} \right)
% \end{aligned}
% \end{equation}
% yields to the desired closed-loop behavior~\cite{van2014port}. Notice that ${H}(\mathbf{x}) = {H}_s(\mathbf{x}) + {H}_u(\mathbf{x})$, i.e.,  the total energy of the system is the sum of the energy of the open-loop dynamics and the energy injected by the controller. \NEWTD{The control $\bfu$ exists as long as the following matching conditions are satisfied:
% \begin{equation}\label{eq:matching_condition}
% \begin{aligned}
% \mathbf{F}_s^{\perp}(\mathbf{x})
% & \left( \left(\mathbf{J}(\mathbf{x}) - \mathbf{R}(\mathbf{x})\right)\frac{\partial {H}(\mathbf{x})}{\partial\mathbf{x}} \right.
% \\
% &-
% \left.\left(\mathbf{J}_s(\mathbf{x}) - \mathbf{R}_s(\mathbf{x})\right)\frac{\partial {H}_s(\mathbf{x})}{\partial\mathbf{x}} \right) = 0,
% \end{aligned}
% \end{equation}
% where $\mathbf{F}_s^{\perp}(\mathbf{x})$ is the maximal-rank left annihilator of $\mathbf{F}_s(\mathbf{x})$, i.e. $\mathbf{F}_s^{\perp}(\mathbf{x})\mathbf{F}_s(\mathbf{x}) = 0$.
% As the control input $\bfu_i$ only affects the robot $i$, the input gain matrix $\mathbf{F}_s(\mathbf{x})$ is block-diagonal: 
% \begin{equation}
%     \bfF_s(\bfx) = \text{diag}\prl
% {\bfF_s^{(1)}(\bfx_1), \ldots, \bfF_s^{(n)}(\bfx_n)},
% \end{equation}
% where $\bfF_s^{(i)}(\bfx_i)$ is the input gain matrix for robot $i$ \TODO{Update notation if the input gain for each robot $i$ is defined in the Problem Statement}. This allows each robot $i$ to evaluate the matching conditions and calculate its control input $\bfu_i$ locally using \eqref{eq:open_loop_intro_controller}. 

% Let $\bfx^*$ be an equilibrium where the Hamiltonian $H(\bfx)$ achieves its minimum. Assuming the matching conditions are satisfied, e.g. when each robot is fully-actuated, i.e. $\bfF_s(\bfx)$ is full-rank, the close-loop system \eqref{eq:closed_loop_intro} is stable around $\bfx^*$ in the sense of Lyapunov with $\partial {H}(\bfx^*)/ \partial \bfx^*  = \mathbf{0}$ and $H(\bfx^*) = 0$ \cite{van2014port}.

% \NA{This is hard to follow for someone who is not familiar with port-Hamiltonian systems. What are the blocks of $\mathbf{F}_s$ and how do they relate to the individual agent dynamics? It might be more intuitive to start the construction from an individual level, talk about the port-Hamiltonian description of the open-loop system and finally design the controller to achieve a desired closed-loop system.}. 
%}
% Besides, we assume that either $\mathbf{F}_s(\mathbf{x})$ is a block-diagonal matrix and $\mathbf{F}_s^{\dagger}(\mathbf{x})$ exists, so it can be computed locally by each robot; or each robot can compute locally the matching conditions that guarantee the existence of $\mathbf{F}_s^{\dagger}(\mathbf{x})$~\cite{yuksel2014reshaping,duong2021hamiltonian}\NA{This is hard to follow for someone who is not familiar with port-Hamiltonian systems. What are the blocks of $\mathbf{F}_s$ and how do they relate to the individual agent dynamics? It might be more intuitive to start the construction from an individual level, talk about the port-Hamiltonian description of the open-loop system and finally design the controller to achieve a desired closed-loop system.}. 


% Observe that, now, the problem of learning the control policy is reduced to finding $\mathbf{J}(\mathbf{x}), \mathbf{R}(\mathbf{x})$ and ${H}(\mathbf{x})$ that solve Eq.~\eqref{eq:prob_def}. The port-Hamiltonian constraints $\mathbf{J}(\mathbf{x}) + \mathbf{J}^T(\mathbf{x})  = \mathbf{0}$,  $\mathbf{R}(\mathbf{x})  \succeq \mathbf{0}$ and ${H}(\mathbf{x})  \geq \mathbf{0}$ must be guaranteed and the robots must be able to compute  $[{H}(\mathbf{x})]_i$ and $[\mathbf{R}(\mathbf{x})]_{ij}, [\mathbf{J}(\mathbf{x})]_{ij}$ $\forall j \in \mathcal{N}_i$ from local information only. By doing so the stability and distributed properties are ensured. Regarding stability, the next result proves that the control policy in Eq.~\eqref{eq:open_loop_intro_controller} guarantees the stability of the closed-loop system under the constraints imposed by the port-Hamiltonian description of the system.

% \NA{The statement of Proposition 1 should include the matching conditions. It is not true that stability can be achieved in general. I am also not sure if Propostion 1 is needed at all since it does not say anything different with respect to what is already known in passivity-based control for (port) Hamiltonian systems. We can state any of the desired properties in the text instead of highlighting as a proposition because the reviewers (at least if I were one) might question the novelty and correctness of Proposition 1.} 

% \begin{proposition}\label{prop:stability}
% The control policy in Eq.~\eqref{eq:open_loop_intro_controller} guarantees the stability of the system in Eq.~\eqref{eq:open_loop_intro} in the Lyapunov sense if $\mathbf{J}(\mathbf{x}) + \mathbf{J}^T(\mathbf{x})  = \mathbf{0}$,  $\mathbf{R}(\mathbf{x})  \succeq \mathbf{0}$ and ${H}(\mathbf{x})  \geq {0}$, and $\partial {H}(\mathbf{x})/ \partial \mathbf{x}  = \mathbf{0}$ 
% % \TD{I am a bit unclear why $\mathbf{J}(\mathbf{x}) = \mathbf{R}(\mathbf{x})  = \mathbf{0}$ at an equilibrium? It does not seem to be satisfied by the closed loop dynamics in Eq. \eqref{eq:closed_loop_Ham}} \ES{that was because the initial architecture couldn't ensure $dH/dx=0$ at equilibrium, so the condition was required to obtain $\dot{V} = 0$ at equilibrium. But the modification of the H architecture now implies $dH/dx = 0$ at equilibrium. Therefore, I have modified the proposition accordingly. Thanks!}
% and ${H}(\mathbf{x}) = {0}$ at equilibrium.
% \end{proposition}
% \begin{proof}
% The closed-loop dynamics in Eq.~\eqref{eq:closed_loop_intro} is obtained by substitution of the control policy of Eq.~\eqref{eq:open_loop_intro_controller} in the open-loop dynamics of Eq.~\eqref{eq:open_loop_intro}. The stability of the closed-loop system is therefore analyzed from Eq.~\eqref{eq:closed_loop_intro}. Without loss of generality, consider $\mathbf{x} = \mathbf{0}$ the desired equilibrium point and $H(\mathbf{x})$ the Lyapunov function candidate such that $H(\mathbf{x}) = 0$ if $\mathbf{x} = \mathbf{0}$ and $H(\mathbf{x}) > 0$ otherwise. The time derivative is
% \begin{equation}\label{eq:Vdot}
% \begin{aligned}
%     \kern -0.3cm\dot{H}(\mathbf{x}) =& \left(\kern -0.1cm\frac{\partial H(\mathbf{x})}{\partial \mathbf{x}}\kern -0.1cm\right)^T\kern -0.3cm\dot{\mathbf{x}} = \\& \left(\kern -0.1cm\frac{\partial H(\mathbf{x})}{\partial \mathbf{x}}\kern -0.1cm\right)^T\kern -0.3cm\left( \mathbf{J}(\mathbf{x}) \kern -0.1cm   - \kern -0.1cm  \mathbf{R}(\mathbf{x})\right)
% \frac{\partial {H}(\mathbf{x})}{\partial\mathbf{x}}. 
% \end{aligned}
% \end{equation}
% Therefore, if $( \mathbf{J}(\mathbf{x})   -   \mathbf{R}(\mathbf{x})) \preceq \mathbf{0}$ and $\frac{\partial {H}(\mathbf{x})}{\partial\mathbf{x}} \neq \mathbf{0}$ for all configurations except the equilibrium, where $\partial {H}(\mathbf{x}) / \partial\mathbf{x} = \mathbf{0}$, then the system is stable in the sense of Lyapunov. First, $  \mathbf{R}(\mathbf{x}) \succeq \mathbf{0}$ by definition of the port-Hamiltonian system. Second, $  \mathbf{J}(\mathbf{x})$ is skew-symmetric by definition of the port-Hamiltonian system, so
% \begin{equation}\label{eq:Jskew}
% \begin{aligned}
%     A =& \frac{\partial H(\mathbf{x})}{\partial \mathbf{x}}^T \mathbf{J}(\mathbf{x}) \frac{\partial H(\mathbf{x})}{\partial \mathbf{x}} \in \mathbb{R} \quad \text{(scalar)},
%     \\
%     A^T =&  \frac{\partial H(\mathbf{x})}{\partial \mathbf{x}}^T \mathbf{J}^T(\mathbf{x}) \frac{\partial H(\mathbf{x})}{\partial \mathbf{x}} = -A.
% \end{aligned}
% \end{equation}
% Therefore, $A = 0$ and $\dot{H}(\mathbf{x}) \leq 0$. If $\partial {H}(\mathbf{x}) / \partial\mathbf{x} = \mathbf{0}$, then the system is stable in the sense of Lyapunov, concluding the proof. 
% \end{proof}

% In turn, the IDA-PBC guarantees stability if the port-Hamiltonian constraints hold and we ensure that, at equilibrium, $\mathbf{J}(\mathbf{x}), \mathbf{R}(\mathbf{x})$ and ${H}(\mathbf{x})$ are zero. Nevertheless, it is important to remark that, to fulfill the conditions in Proposition~\ref{prop:stability} \textbf{and} achieve the task, the equilibrium of the observed and learned closed-loop dynamics must be the same\NA{This is vague. We did not define what ``an equilibrium'' means and how the equilibria of the learned and demonstrated closed-loop systems correspond. We should either remove this or make it more precise by introducing the Hamiltonian $H^*(\mathbf{x})$ resulting from the true policy and discussing the relationship between $\arg\min_{\mathbf{x}} H^*(\mathbf{x})$ and $\arg\min_{\mathbf{x}} H(\mathbf{x})$.}; otherwise, despite converging, there is no guarantee that the learned control policy drives the system towards the correct equilibrium. Besides, if the port-Hamiltonian terms are computed in a distributed fashion, then the learning problem is successfully moved from an unstructured learning problem within a large class of control policies to a structured learning problem within a tighter class of control policies that guarantee stability and a distributed architecture. In the next Subsection we propose a solution to learn $\mathbf{R}(\mathbf{x}), \mathbf{J}(\mathbf{x})$ and ${H}(\mathbf{x})$ such that they respect both the port-Hamiltonian, stability and distributed constraints. 

\begin{example}\label{example:portHamiltonian}
The closed-loop dynamics for the flocking problem in Example~\ref{example:flocking_controller} are:
%
\begin{equation}\label{eq:closed_loop_new}
\begin{aligned}
        \dot{{\mathbf{p}}} &= {\mathbf{v}},\quad
        \dot{{\mathbf{v}}} = -\frac{\partial {U}_{\bftheta}({\mathbf{p}})}{\partial{\mathbf{p}}} - \mathbf{D}_{\bftheta}({\mathbf{p}}){\mathbf{v}}, \\\hbox{ with }
        \frac{\partial {U}_{\bftheta}({\mathbf{p}})}{\partial{\mathbf{p}}_i}  &= c_1{\mathbf{p}}_i + \sum_{j \in \mathcal{N}_i^1}  \phi(||{\mathbf{p}}_{j}-{\mathbf{p}}_i||_{\sigma})\mathbf{n}_{ij},
        \\
         [\mathbf{D}_{\bftheta}({\mathbf{p}})]_{ij}  &=  \left(  c_2 [\mathbf{I}_n]_{ij}  +  \rho \left(||{\mathbf{p}}_{j}-{\mathbf{p}}_i||_{\sigma}/\tau\right) \right) \mathbf{I}_m.
\end{aligned}
\end{equation}
%
In port-Hamiltonian terms, ${H}_{s}(\bfx) = \frac{1}{2}{\mathbf{v}}^\top{\mathbf{v}}$, $\bfR_s = \mathbf{0}$, $\mathbf{F}_s(\mathbf{x}) = [\mathbf{0}, \mathbf{I}_m]^\top$, 
% \begin{equation}\label{eq:closed_loop_Ham}
%         \kern -0.4cm\begin{pmatrix}
%         \dot{{\mathbf{p}}} \\ \dot{{\mathbf{v}}}
%         \end{pmatrix}
%         = \prl{\bfJ - \bfR} \begin{pmatrix}
%         \frac{\partial {H}({\mathbf{p}}, {\mathbf{v}})}{\partial{\mathbf{p}}}\\ \frac{\partial {H}({\mathbf{p}}, {\mathbf{v}})}{\partial{\mathbf{v}}}
%         \end{pmatrix},
% \end{equation}
$\bfJ_{s}(\bfx) = \bfJ_{\bftheta}(\bfx) =          \begin{pmatrix}
        \mathbf{0} & \kern -0.2cm \mathbf{I}_n\\ -\mathbf{I}_n & \kern -0.2cm\mathbf{0}
        \end{pmatrix}$, $\bfR_{\bftheta}(\bfx) =          \begin{pmatrix}
        \mathbf{0} &  \mathbf{0}\\ \mathbf{0} &  \mathbf{D}_{\bftheta}({\mathbf{p}})
        \end{pmatrix}$, and ${H}_{\bftheta}(\bfx) = U_{\bftheta}({\mathbf{p}}) + \frac{1}{2}{\mathbf{v}}^\top{\mathbf{v}}$.
% In this example, learning $\mathbf{D}({\mathbf{p}})$ and ${U}({\mathbf{p}})$ is equivalent to learning the control policy that captures the flocking interactions.
\end{example}


% \begin{equation}\label{eq:open_loop}
% \begin{aligned}
%         \dot{\mathbf{v}} &= - \mathcal{F}(\mathbf{x})\mathcal{F}_u^T(\mathbf{x})\frac{\partial \mathcal{H}_u(\mathbf{x})}{\partial \mathbf{x}}
% \\
% &= \left(\mathcal{J}_u(\mathbf{x}) - \mathcal{R}_u(\mathbf{x})\right)\frac{\partial \mathcal{H}_u(\mathbf{x})}{\partial\mathbf{x}}.
% \end{aligned}
% \end{equation}
% If $\mathcal{F}_u = \mathbf{I}$, $\mathcal{J}_u = \mathbf{0}$ and $\mathcal{F} = \mathcal{R}_u$, then Eq.~\eqref{eq:open_loop} holds.
% % \begin{equation}\label{eq:open_loop_intro_controller2}
% %         \mathbf{u} = -\mathcal{F}_s^{\dagger}\left(\left(\mathcal{J}_s(\mathbf{x}) - \mathcal{R}_s(\mathbf{x})\right)\frac{\partial \mathcal{H}_s(\mathbf{x})}{\partial\mathbf{x}}\left(\frac{\partial \mathcal{H}_u(\mathbf{x})}{\partial\mathbf{x}}\right)^{\ddagger} + \left(\mathcal{J}(\mathbf{x}) - \mathcal{R}(\mathbf{x})\right)\frac{\partial \mathcal{H}(\mathbf{x})}{\partial\mathbf{x}}\left(\frac{\partial \mathcal{H}_u(\mathbf{x})}{\partial\mathbf{x}}\right)^{\ddagger}\right)
% % \end{equation}
% The interconnection of two port-Hamiltonian systems is also a port-Hamiltonian system~\cite{shaft2004port}, with total energy $\mathcal{H}(\mathbf{x}) = \frac{1}{2}\mathbf{v}^T\mathbf{v} + \mathcal{H}_u(\mathbf{x})$. Therefore, 

% Note that $\partial \mathcal{H}(\mathbf{x}) / \partial\mathbf{v} = \mathbf{v}$, which implies that $\mathcal{H}_u(\mathbf{x}) = \mathcal{H}_u(\mathbf{p})$ and therefore $\partial \mathcal{H}(\mathbf{x}) / \partial\mathbf{p} = \partial \mathcal{H}_u(\mathbf{p}) / \partial\mathbf{p}$. 
 

% Last but not least, if constraints $\mathcal{R}(\mathbf{x}) \succeq \mathbf{0}$ and $\mathcal{H}(\mathbf{x}) \geq 0$ are enforced, then the system is stable, and so the control policy does not destabilize the system by construction.





% \ES{At this point of the research, we might need to discuss what do we really want to propose as solution. Some tips: (i) If the solution (Steps 1 and 2) receives, as input, the whole state, then even if we use the Boolean Laplacian to constraint the training, then the policy is not distributed. On the other hand, Step 3 yields to a distributed policy, so in a realistic deployment, only Step 3 is affordable. Therefore, Steps 1 and 2 remain an identification solution, while Step 3 obtains a really implementable policy; (ii) Step 1 is a bit unrealistic because we could obtain a $\tau$ that does not correspond to the actual messages a robot is receiving during deployment; (iii) If the solution works online, then the loss function should reflect not only the error between predicted and actual, but also the control objective itself; (iv) for sure that the solution can be embedded in a RL framework (see PettingZoo slides), but this may be a future step. Afterwards, we could use Isaac Gym} 

\subsection{Learning Distributed Multi-Robot Interactions}\label{subsec:LEMURS}

We seek to learn control policies that scale with the number of robots, handle time-varying communications and guarantee the port-Hamiltonian constraints. To do so, we first derive conditions on $\mathbf{J}_{\bftheta}(\mathbf{x})$, $\mathbf{R}_{\bftheta}(\mathbf{x})$ and ${H}_{\bftheta}(\mathbf{x})$, which are the terms to be learned from task demonstrations. Then, we develop a novel architecture based on self-attention and neural ordinary differential equations to ensure that the learned control policies guarantee these conditions.

To respect the team topology, we first impose  $\mathbf{J}_{\bftheta}(\mathbf{x})$ and $\mathbf{R}_{\bftheta}(\mathbf{x})$ to be block-sparse, 
\begin{equation} 
\label{eq:JRH_conditions1}
        [\mathbf{J}_{\bftheta}(\mathbf{x})]_{ij} =
        [\mathbf{R}_{\bftheta}(\mathbf{x})]_{ij} = \mathbf{0}, \quad \forall j \notin \calN_i^k,
\end{equation}
% and forcing the rest of the blocks to depend only on $\bfx_{\calN_i^{2k}}$,
% \begin{equation} 
% \label{eq:JRH_conditions2}
%         \kern-8 pt [\mathbf{J}_{\bftheta}(\mathbf{x})]_{ij} = \bfJ_{\bm\theta}^{(j)}(\bfx_{\calN_j^{2k}}),\;
%         [\mathbf{R}_{\bftheta}(\mathbf{x})]_{ij} = \bfR_{\bm\theta}^{(j)}(\bfx_{\calN_j^{2k}}), \forall j \in \calN_i^k.
% \end{equation}
Moreover, 
%To respect the team topology, 
we require that the desired Hamiltonian factorizes over $k$-hop neighborhoods:
%In Sec.~\ref{subsec:portHamiltonian}, we reduce   problem~\eqref{eq:prob_def} to learning $\mathbf{J}(\mathbf{x})$, $\mathbf{R}(\mathbf{x})$ and ${H}(\mathbf{x})$ from data. We first define the desired Hamiltonian as a function of the $k-$hop neighbors, such that:
\begin{equation} \label{eq:individual_Hi}
        H_{\bftheta}(\mathbf{x}) = \sum_{i=0}^n H_{\bftheta}^{(i)}(\bfx_{\calN_i^{k}}).
\end{equation}
% \begin{equation} \label{eq:individual_Hi}
%         H_{\bftheta}(\mathbf{x}) = \sum_{i=0}^n H_{\bftheta}^{(i)}(\mathbf{x}_i, \{\mathbf{x}_j\}_{j\in{\mathcal{N}^k_i}}) =: \sum_{i=0}^n H_{\bftheta}^{(i,k)}.
% \end{equation}
The factorization in \eqref{eq:individual_Hi} ensures that each robot $i$ can calculate  $\partial H_{\bftheta}(\bfx)/\partial \mathbf{x}_i = \sum_{j\in \calN_i^k}{\partial H^{(j)}_{\bftheta}(\bfx_{\calN_j^{k}})/\partial \mathbf{x}_i}$ by gathering $\partial H^{(j)}_{\bftheta}(\bfx_{\calN_j^{k}})/\partial \mathbf{x}_i$ from its $k$-hop neighbors $j$.
% $\frac{\partial}{\partial \mathbf{x}_j}\frac{\partial H_{\bftheta}(\mathbf{x})}{\partial \mathbf{x}_i}~=~0,\quad \forall j \notin \mathcal{N}^{k+1}_i$, i.e. $\frac{\partial H_{\bftheta}(\mathbf{x})}{\partial \mathbf{x}_i}$
%
% \begin{equation} \label{eq:partials}
%         \frac{\partial}{\partial \mathbf{x}_j}\frac{\partial H_{\bftheta}(\mathbf{x})}{\partial \mathbf{x}_i} = 0,\quad \forall j \notin \mathcal{N}^{k+1}_i,
% \end{equation}
% which means that the partial of the joint Hamiltonian with respect to robot $i$ depends on the state information from at most its $(k+1)$-hop neighbors. For instance, a $1$-hop distributed policy requires that $H_{\bftheta}^{(i,0)}$ only depends on $\mathbf{x}_i$, i.e., the $0$-hop neighbors. 
% Besides, we require  $\mathbf{J}_{\bftheta}(\mathbf{x})$, $\mathbf{R}_{\bftheta}(\mathbf{x})$ to be block-sparse and such that each $(i,j)-$block is computed from neighboring information: %
% \begin{equation} 
% \label{eq:JRH_conditions}\kern -10pt
% \begin{aligned}\relax 
%         [\mathbf{J}_{\bftheta}(\mathbf{x})]_{ij} =& 
%         [\mathbf{R}_{\bftheta}(\mathbf{x})]_{ij} = \mathbf{0}, \quad \forall j \notin \calN_i^k,
%         \\
%         [\mathbf{J}_{\bftheta}(\mathbf{x})]_{ij} =:&  \mathbf{J}_{\bftheta}^{(i,j)}(\mathbf{x}_i, \{\mathbf{x}_j\}_{j\in{\mathcal{N}^k_i}}) =: \mathbf{J}_{\bftheta}^{(i,j, k)}, \quad \kern -5pt \forall j \in \calN_i^k,
%         \\
%         [\mathbf{R}_{\bftheta}(\mathbf{x})]_{ij} =:&  \mathbf{R}_{\bftheta}^{(i,j)}(\mathbf{x}_i, \{\mathbf{x}_j\}_{j\in{\mathcal{N}^k_i}}) =: \mathbf{R}_{\bftheta}^{(i,j, k)}, \quad \kern -5pt \forall j \in \calN_i^k.
% \end{aligned}

% \end{equation}
Then, the control policy $\bfpi_{\bftheta}$ of robot $i$ becomes:
% For brevity, let $\mathbf{x}^a_i = [\mathbf{x}_{i}^T, \mathbf{x}_{j_1}^T, \mathbf{x}_{j_2}^T, \hdots, \mathbf{x}^T_{j_{|\mathcal{N}_i|}}]^T.$ To make the controller \eqref{eq:open_loop_intro_controller_ind} distributed, robot $i$ must be able to calculate $\bfu_i$ from local information, i.e., calculating $[\mathbf{J}(\mathbf{x})]_{ij}$,  $[\mathbf{R}(\mathbf{x})]_{ij}$, and $\partial H/\partial \bfx_i$ only from $\mathbf{x}^a_i$. Specifically, if robot $j$ is a neighbor of robot $i$, i.e. $j \in \calN_i$, the energy exchange and dissipation only depends on $\bfx_a^i$. 
% \begin{gather} \label{eq:individual_JR}
%         [\mathbf{J}(\mathbf{x})]_{ij} = \mathbf{J}^{(ij)}(\mathbf{x}^a_i), \hbox{ }
%         [\mathbf{R}(\mathbf{x})]_{ij} = \mathbf{R}^{(ij)}(\mathbf{x}^a_i) \hbox{ } \forall i \in \calV, j \in \calN_i.
% \end{gather}
% Otherwise, there is no such energy exchange or dissipation:
% Meanwhile, we model the desired Hamiltonian of system \eqref{eq:closed_loop_intro} as the sum of $n$ desired individual Hamiltonian $H^{(i)}(\mathbf{x}^a_i), i \in \calV$. Each desired Hamiltonian $H^{(i)}(\mathbf{x}^a_i)$ corresponds to the total energy of robot $i$ and only depends on its local information $\bfx^a_i$:
% so that each robot can compute its own Hamiltonian functions from local information and $\partial H(\bfx)/\partial \bfx_i$ only depends on $\bfx^a_i$, \TD{Is it true? Since $H^{(j)}$ can also contains $\bfx_i$ if $j \in \calN_i$, meaning $\partial H / \partial \bfx_i = \sum_{j \in \calN_i \cup \{i\}} \partial H^{(j)}(\bfx^a_j)/\partial \bfx_i \neq \partial H^{(i)}(\bfx_i^a) / \partial \bfx_i$. Are we approximating $\partial H / \partial \bfx_i$ by $\partial H^{(i)} / \partial \bfx_i$ ? If so, I think we should clarify and tone down stability of closed-loop system more since the approximation might break the stability.}
\begin{align}
\kern -5pt \mathbf{u}_i &= \mathbf{F}_s^{(i)\dagger}(\mathbf{x}_i)
\left( \sum_{j \in \calN_i^k}\kern -0.2cm \left([\mathbf{J}_{\bftheta}(\mathbf{x})]_{ij} \kern -0.1cm-\kern -0.1cm [\mathbf{R}_{\bftheta}(\mathbf{x})]_{ij}\right)\frac{\partial H_{\bftheta}(\mathbf{x})}{\partial \mathbf{x}_j}  \right. 
\notag\\
& \qquad \qquad \left. -\left(\mathbf{J}_s^{(i)}(\mathbf{x}_i) - \mathbf{R}_s^{(i)}(\mathbf{x}_i)\right)\frac{\partial {H}_s^{(i)}(\mathbf{x})}{\partial\mathbf{x}_i} \right). \label{eq:open_loop_intro_controller_ind_distributed}
\end{align}
% \begin{equation}\label{eq:open_loop_intro_controller_ind_distributed}
% \begin{aligned}
% \kern -5pt \mathbf{u}_i &= \mathbf{F}_s^{\dagger}(\mathbf{x}_i)
% \left( \sum_{j \in \calN_i^k \cup \{i\}}\kern -0.3cm \left(\mathbf{J}_{\bftheta}^{(i,j,k)} \kern -0.1cm-\kern -0.1cm \mathbf{R}_{\bftheta}^{(i,j,k)}\right)\frac{\partial H_{\bftheta}(\mathbf{x})}{\partial \mathbf{x}_j}  \right. 
% \\
% & \qquad \qquad \left. -\left(\mathbf{J}_s^{(i)}(\mathbf{x}_i) - \mathbf{R}_s^{(i)}(\mathbf{x}_i)\right)\frac{\partial {H}_s^{(i)}(\mathbf{x})}{\partial\mathbf{x}_i} \right).
% \end{aligned}
% \end{equation}
% leading to robot $i$'s closed-loop dynamics:\NA{It is not necessary to provide the closed-loop dynamics of an individual agent. Plus these are true only if the matching condition holds.}
% \begin{equation}\label{eq:individual_dynamics}
%     \dot{\mathbf{x}}_i = \sum_{j \in \mathcal{N}^k_i \cup \{i\}}\left(\mathbf{J}^{(i,j,k)} - \mathbf{R}^{(i,j,k)}\right)\frac{\partial H(\mathbf{x})}{\partial \mathbf{x}_j}.
% \end{equation}
Imposing the requirements in \eqref{eq:JRH_conditions1}-\eqref{eq:individual_Hi} is a first step towards making the control policy in \eqref{eq:open_loop_intro_controller_ind_distributed} distributed. Note that the terms $[\mathbf{J}_{\bftheta}(\mathbf{x})]_{ij}$ and $[\mathbf{R}_{\bftheta}(\mathbf{x})]_{ij}$ might still depend on the joint state $\bfx$ even if $j \in \calN_i^k$. We discuss how to remove this dependence next and achieve a similar factorization as \eqref{eq:individual_Hi}.

%Later on, we develop how to remove the dependencies of the learned quantities with states outside the neighborhood $\mathcal{N}_i^k$. In the following, we omit the dependencies with $\bfx$ for notation compactness.

% We assume that any of the three options hold\NA{What is this sentence saying?}.

% each neighboring robot $j\in\calN_i$ have to send its information ,  to robot $i$, which in turns, needs the states of robot $j$'s neighbor $\bfx_k, k \in \calN_j$. It implies that our control policy computation requires a 2-hop communications on the graph $\calG$ among the robots.

% To satisfy the requirements in \eqref{eq:JRH_conditions} for a distributed control policy, we define the desired Hamiltonian of system \eqref{eq:closed_loop_intro} as the sum of $n$ desired individual Hamiltonian $H^{(i)}(\mathbf{x}^a_i), i \in \calV$. Each desired Hamiltonian $H^{(i)}(\mathbf{x}^a_i)$ corresponds to the total energy of robot $i$ and only depends on its local information $\bfx^a_i$:

% \begin{equation} \label{eq:individual_terms}
%     \begin{aligned}
%         H(\mathbf{x}) =& \sum_{i=0}^n H^{(i)}(\mathbf{x}^a_i) \\
%         [\mathbf{J}(\mathbf{x})]_{i} =& \mathbf{J}^{(i)}(\mathbf{x}^a_i), \quad \forall i\\
%         [\mathbf{R}(\mathbf{x})]_{i} =& \mathbf{R}^{(i)}(\mathbf{x}^a_i), \quad \forall i
%     \end{aligned}
% \end{equation}
% \begin{gather} \label{eq:individual_terms}
%         H(\mathbf{x}) = \sum_{i=0}^n H^{(i)}(\mathbf{x}^a_i), \\
%         [\mathbf{J}(\mathbf{x})]_{i} = \mathbf{J}^{(i)}(\mathbf{x}^a_i), \hbox{ }
%         [\mathbf{R}(\mathbf{x})]_{i} = \mathbf{R}^{(i)}(\mathbf{x}^a_i) \hbox{ } \forall i
% \end{gather}
% so each robot can compute its own Hamiltonian functions from local information. 
% \begin{equation}\label{eq:open_loop_intro_controller_ind}
% \begin{aligned}
% \kern -0.2cm \mathbf{u}_i &= (\mathbf{F}_s^{(i)}(\mathbf{x}_i))^{\dagger}
% \left((\mathbf{J}^{(i)}(\mathbf{x}_i^a) - \mathbf{R}^{(i)}(\mathbf{x}_i^a) \frac{\partial H^{(i)}(\mathbf{x}_i^a)}{\partial\mathbf{x}_i^a}-\right.
% \\
% & \qquad \qquad \qquad \left.(\mathbf{J}_s^{(i)}(\mathbf{x}_i) - \mathbf{R}_s^{(i)}(\mathbf{x}_i)) \frac{\partial {H}_s^{(i)}(\mathbf{x}_i)}{\partial\mathbf{x}_i}\right).
% \end{aligned}
% \end{equation}
% From Eqs.~\eqref{eq:open_loop_intro_individual} and \eqref{eq:open_loop_intro_controller_ind}, the control policy yields to the robot $i$ closed-loop dynamics 
% \begin{equation}\label{eq:individual_dynamics}
%     \dot{\mathbf{x}}_i = \sum_{j \in \mathcal{N}_i \cup \{i\}}([\mathbf{J}(\mathbf{x}_i^a)]_{ij}-[\mathbf{R}(\mathbf{x}_i^a)]_{ij})\frac{\partial H(\mathbf{x})}{\partial \mathbf{x}_j}.
% \end{equation}
\subsubsection{Modeling robot interactions using self-attention}
\label{subsubsec:sa_architecture_JRH}
We model $[\mathbf{J}_{\bftheta}]_{ij}, [\mathbf{R}_{\bftheta}]_{ij}$, and $H_{\bftheta}^{(i)}$ in
%We model the terms $\bfJ_{\bftheta}^{(i,j,k)}, \bfR_{\bftheta}^{(i,j,k)}$, $H_{\bftheta}^{(i,k)}$ in 
Eq.~\eqref{eq:open_loop_intro_controller_ind_distributed} with the parameters $\bftheta$ shared across the robots, so that the team can handle time-varying communication graphs.
% Besides, it is desirable to find a way of learning  $[\mathbf{J}(\mathbf{x})]_{ij}, [\mathbf{R}(\mathbf{x})]_{ij}$ and $\frac{\partial H_i(\mathbf{x})}{\partial \mathbf{x}_j}$ such that, if they are implemented in a team with a time-varying number of robots\NA{Save this for the experiments section. So far our problem formulation has not considered $n$} or the graph topology changes with time, then the task is still accomplished. 
Specifically, we propose a novel architecture 
%of  $\bfJ_{\bftheta}^{(i,j,k)}, \bfR_{\bftheta}^{(i,j,k)}$, $H_{\bftheta}^{(i,k)}$ 
based on self-attention~\cite{vaswani2017attention}. Self-attention layers extract the relationships among the inputs of a sequence by calculating the importance associated to each input using an attention map. The length of the sequences can vary as the number of parameters of the self-attention is constant with the number of inputs. Our key idea is to consider the self and neighboring information as the sequence, where each neighbor's information is an input. 
%Then, the attention map is used to calculate the importance associated to each input.
% :\NA{The equation below does not appear necessary.}
% \begin{equation}\label{eq:individual_dynamics_parameters}
%     \dot{\mathbf{x}}_i = \kern -0.2cm \sum_{j \in \mathcal{N}^k_i \cup \{i\}}\kern -0.2cm \left(\mathbf{J}^{(i,j,k)}(\bm{\theta_J}) - \mathbf{R}^{(i,j,k)}(\bm{\theta_R})\right)\frac{\partial H(\mathbf{x}, \bm{\theta}_H)}{\partial \mathbf{x}_j}.
% \end{equation}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Images/FigureArchitecture.png}
    \caption{\small{Proposed architecture for LEMURS. Robot $i$ receives information from its neighbors. Then, the self-attention module processes the data to obtain the port-Hamiltonian terms. With this information, robot $i$ computes the learned control policy through an ordinary differential equation solver.}}
    \label{fig:architecture}
\end{figure}

More precisely, to learn
$[\mathbf{R}_{\bftheta}]_{ij},$
%$\mathbf{R}_{\bftheta}^{(i,j,k)}$,
robot $i$ will use, at instant $t$, the states $\bfx_j$ from all $k-$hop neighbors $j \in \mathcal{N}^k_i$, which are concatenated as:
\begin{equation} \label{eq:concatenated_neighbors}
    \mathbf{X}_i^0 = [\mathbf{x}_{i},     \mathbf{x}_{j_1}, \mathbf{x}_{j_2}, \hdots, \mathbf{x}_{j_{\left|\mathcal{N}_i^k\right|}}] \in \bbR^{n_x \times (|\calN_i^k| + 1)}.
\end{equation}
For each layer $w=1,\hdots, W$, we define:
\begin{align}\label{eq:selfattention}
        % &\kern -5pt\mathbf{X}_i^1 = [\mathbf{x}_{i},     \mathbf{x}_{j_1}, \mathbf{x}_{j_2}, \hdots, \mathbf{x}_{j_{\left|\mathcal{N}_i^k\right|}}].
        % \\
        % &\kern -0.2cm\kern -5pt\text{ For each layer }w=1,\hdots, W, \text{ we define:}
        % \\
        &\kern -0.2cm \mathbf{Q}_i^w =  \mathbf{A}^w_{Q,\mathbf{R}}{\mathbf{X}}_i^w, \hbox{ } \mathbf{K}_i^w = \mathbf{A}^w_{K,\mathbf{R} }\mathbf{X}_i^w, \hbox{ } \mathbf{V}_i^w = \mathbf{A}^w_{V,\mathbf{R}}\mathbf{X}_i^w, 
    \\
    &\kern -0.2cm\mathbf{Y}_i^w = \gamma\left(\mathsf{softmax}\left(\frac{\beta(\mathbf{Q}^w_i)\beta((\mathbf{K}_i^w)^{\top})}{\sqrt{|\mathcal{N}_i|}}\right) \beta(\mathbf{V}_i^w)\right),
    \\
    &\kern -0.2cm\mathbf{X}_i^w = \alpha(\mathbf{A}^w_{Z, \mathbf{R}}{\mathbf{Y}}_i^w),\label{eq:selfattention2}   
\end{align}
where $W$ is the number of self-attention layers; $\mathbf{A}^w_{Q, \mathbf{R}}, \mathbf{A}^w_{K, \mathbf{R}}, \mathbf{A}^w_{V, \mathbf{R}} \in \mathbb{R}^{r_w \times h_w}$ and $\mathbf{A}^w_{Z, \mathbf{R}} \in \mathbb{R}^{d_w \times r_w}$ for $w =1, \ldots, W$ are matrices to be learned and shared across robots; and $h_w, r_w, d_w>0$, with $d_W = n_x^2$ and $h_1 = n_x$ for valid matrix multiplications. The size of $\mathbf{A}^w_{Q, \mathbf{R}}, \mathbf{A}^w_{K, \mathbf{R}}, \mathbf{A}^w_{V, \mathbf{R}}$ does not depend on the number of robots, so robot $i$ can deal with time-varying neighbors. Nonlinear activation functions $\beta(\cdot)$, $\gamma(\cdot)$ and $\alpha(\cdot)$ account for potential nonlinearities. 
% \TD{Maybe I missed something here but how does $n$ appears here while $\mathbf{X}_i \in \mathbb{R}^{n_x \times |\mathcal{N}_i + 1|}$?} \ES{Typo, corrected}.
Then, $[\mathbf{R}_{\bftheta}]_{ij}$ is constructed as a weighted matrix that models the interactions of robot $i$ with its neighbors, and a diagonal positive semidefinite matrix that accounts for the self-interactions:
\begin{gather}\label{eq:Restimate}
    \begin{aligned}
    \mathbf{Z}_{ij}^R =& \mathsf{vec}^{-1}(\mathbf{x}_{ij}^W)
    \\
   [\mathbf{R}_{\bftheta}]_{ij} =& -({\mathbf{Z}}_{ij}^{R}+{\mathbf{Z}}_{ji}^{R}), \quad  \forall j \in \mathcal{N}^k_i\backslash \{i\},
    \\
    [\mathbf{R}_{\bftheta}]_{ii} =& {\mathbf{Z}}_{ii}^{R} +  \sum_{j \in \mathcal{N}_i^k \backslash \{i\}}  ({\mathbf{Z}}_{ij}^{R}+{\mathbf{Z}}_{ji}^{R}),
    \end{aligned}
\end{gather}
where $\mathbf{x}_{ij}^W$ is the column $\mathbf{x}_j$ that corresponds to neighbor $j$ in $\mathbf{X}_i^W$,  $\mathsf{vec}^{-1}(\cdot)$ is the operator that reshapes the $d_W \times 1$ vector to a $n_x \times n_x$ matrix.
This way, $[\mathbf{R}_{\bftheta}]_{ij}$ is positive semidefinite by design.
% The steps in~\eqref{eq:Restimate} ensure that 
% %$\hat{\mathbf{R}}(\mathbf{x}) \in \mathsf {wspace}(\mathbf{L})$; this implies that 
% ${\mathbf{R}}(\mathbf{x}) \succeq \mathbf{0}$ by construction. 

% a row vector ${\mathbf{a}}_i$ and a scalar ${{a}}_i$ are computed
% \begin{equation}\label{eq:adjacency}
% \begin{aligned}
%     \relax[{\mathbf{a}}_i]_{j} =& \gamma((\mathbf{w}^R_{j})^T \mathbf{y}^R_i)^2  \hbox{ } \forall j \in \mathcal{N}_i, \hbox{ and $0$ otherwise},
%     \\
%     {{a}}_i =& \gamma((\mathbf{w}^R_{i})^T\mathbf{y}_i)^2.
% \end{aligned}
% \end{equation}
% Here, $\gamma(\cdot)$ is a nonlinear activation function. Finally,
%  . 
% Its skew-symmetry is maintained by enforcing $$\mathbf{J}^{(i,j,k)}(\bm{\theta_J}) = -  \mathbf{J}^{(j,i,k)}(\bm{\theta_J})\quad \forall j \in \mathcal{N}_i^k.$$ 

To construct $[\mathbf{J}_{\bftheta}]_{ij}$, we follow the same steps \eqref{eq:selfattention}-\eqref{eq:selfattention2}, with parameters $\mathbf{A}^w_{Q, \mathbf{J}}, \mathbf{A}^w_{K, \mathbf{J}}, \mathbf{A}^w_{V, \mathbf{J}}$ and $\mathbf{A}^w_{Z, \mathbf{J}}$, to obtain encodings $\bfZ_{ij}^J$. Due to the undirected communication between robots $i$ and $j$, we enforce the skew-symmetry of $\bfJ_\bftheta$ by:
%construct $\mathbf{J}^{(i,j,k)}_{\bftheta}$ as follows, enforcing its skew-symmetry: 
\begin{equation}\label{eq:Jestimate}
    [\mathbf{J}_{\bftheta}]_{ij} = {\mathbf{Z}}_{ij}^{J}-{\mathbf{Z}}_{ji}^{J} \quad \forall j \in \mathcal{N}^k_i.
\end{equation}

% Regarding $\partial H_{\bftheta}(\mathbf{x})/\partial \mathbf{x}_j$,  similar steps can be followed. Each robot computes 
For each robot $i$, we construct $H^{(i)}_{\bftheta}$ as follows:
\begin{equation}\label{eq:Hestimate}
H^{(i)}_{\bftheta} = (\mathsf{vec}(\mathbf{X}_i^0))^{\top} \mathbf{M}_{\bftheta}^{(i)}(\mathbf{X}_i^0)(\mathsf{vec}(\mathbf{X}_i^0)) + {U}_{\bftheta}^{(i)}(\mathbf{X}_i^0),
% \begin{aligned}
%   H^{(i,k)}_{\bftheta} =& (\mathsf{vec}(\mathbf{X}_i))^{\top} \mathbf{M}_{\bftheta}^{(i)}(\mathbf{X}_i)(\mathsf{vec}(\mathbf{X}_i)) + {U}_{\bftheta}^{(i)}(\mathbf{X}_i), \hbox{ } \text{where}
%     \\
%     &\mathsf{diag}(\mathbf{M}_{\bftheta}^{(i)}(\mathbf{X}_i)) = \mathbf{1}^{\top}\mathbf{Z}^M_i, \quad \text{and}
%     \\
%     &{U}_{\bftheta}^{(i)}(\mathbf{X}_i) = \mathbf{1}^{\top}\mathbf{Z}^U_i\mathbf{1}.
% \end{aligned}
\end{equation}
where the first term $(\mathsf{vec}(\mathbf{X}_i^0))^{\top} \mathbf{M}_{\bftheta}^{(i)}(\mathbf{X}_i^0)(\mathsf{vec}(\mathbf{X}_i^0))$ is a kinetic-like energy function with $\mathbf{M}_{\bftheta}^{(i)}(\mathbf{X}_i^0) = \diag( \mathbf{1}^{\top}\mathbf{Z}^M_i)$, and the second term ${U}_{\bftheta}^{(i)}(\mathbf{X}_i^0)$ is a potential energy function with ${U}_{\bftheta}^{(i)}(\mathbf{X}_i^0) = \mathbf{1}^{\top}\mathbf{Z}^U_i\mathbf{1}$.
The encodings $\mathbf{Z}^M_i$ and $\mathbf{Z}^U_i$ are calculated using the same steps ~\eqref{eq:selfattention}-\eqref{eq:selfattention2}, with parameters  $\mathbf{A}^w_{Q, \mathbf{M}}, \mathbf{A}^w_{K, \mathbf{M}}, \mathbf{A}^w_{V, \mathbf{M}}$ and $\mathbf{A}^w_{Z, \mathbf{M}}$, and $\mathbf{A}^w_{Q, U}, \mathbf{A}^w_{K, U}, \mathbf{A}^w_{V, U}$ and $\mathbf{A}^w_{U}$, respectively.
%To calculate $\mathbf{Z}^M_i$ and $\mathbf{Z}^U_i$, steps~\eqref{eq:selfattention}-\eqref{eq:selfattention2} are followed, with parameters  $\mathbf{A}^w_{Q, \mathbf{M}}, \mathbf{A}^w_{K, \mathbf{M}}, \mathbf{A}^w_{V, \mathbf{M}}$ and $\mathbf{A}^w_{Z, \mathbf{M}}$, and $\mathbf{A}^w_{Q, U}, \mathbf{A}^w_{K, U}, \mathbf{A}^w_{V, U}$ and $\mathbf{A}^w_{U}$.
With $H^{(i)}_{\bftheta}$, we  obtain $\frac{\partial H^{(i)}_{\bftheta}}{\partial \mathbf{x}_j}$   $\forall j \in \mathcal{N}^k_{i}$ and compute  $\frac{\partial H_{\bftheta}}{\partial \bfx_i} = \sum_{j \in \mathcal{N}_i^k } \frac{\partial H^{(j)}}{\partial \bfx_i}$. 

% Importantly,~\eqref{eq:Hestimate} implies that, if $\mathbf{X}_i = \mathbf{0}$ \TD{In Sec 3A, we talked about stability around $\bfx^*$ with  $\partial {H}(\mathbf{x})/ \partial \mathbf{x} = 0$ and ${H}(\mathbf{x}) = 0$. Here, it seems like $\bfx^* = 0$. Should we clarify here that the state can be offset by $\bfx^*$ to move the equilibrium to $0$? This is more consistent with the offset network input in the Appendix.}, then both $\partial {H}(\mathbf{x})/ \partial \mathbf{x}$ and ${H}(\mathbf{x})$ are zero, which fulfills the stability requirements.
% \TD{Why }\ES{Typo from previous versions, corrected}.

\subsubsection{Learning distributed control policies using neural ODE networks}
Let
$\mathsf{SA}(\mathbf{X}_i^0,\bm{\theta})$ denote the operations from~\eqref{eq:selfattention} to~\eqref{eq:Hestimate} with $$\bm{\theta} = \{ \{\mathbf{A}^w_{Q, k}, \mathbf{A}^w_{K, k}, \mathbf{A}^w_{V, k}, \mathbf{A}^w_{Z, k}\}_{w=1}^{w=W}\}_{k=\mathbf{R,J,M},U}.$$
To address Problem \eqref{eq:prob_def}, we use a neural ODE network \cite{chen2018neural} whose structure respects the continuous-time dynamics in \eqref{eq:open_loop_intro_individual}. To calculate the loss $\mathcal{L}({\mathcal{D}},\bar{\mathcal{D}})$ in \eqref{eq:loss_function}, for each trajectory $l$ of robot $i$, $\{\bfx_i^l(rT)\}_{r = 0}^K$ in the data, we solve an ODE:
%
\begin{equation}
\dot{\bfx}^l_i = \bff_i(\bfx^l_i, \bfpi_\bftheta;\bftheta), \quad \bfx^l_i(0) = \bar{\bfx}^l_i(0),
\end{equation}
%
using an ODE solver to obtain a predicted state $\bfx_i^l(rT)$ for $i \in \calV, l = 0, \ldots, L$: 
\begin{equation}
\bfx^l_i = \mathsf{ODESolver}\prl{\bfx^l_i(0), \bff_i, rT; \bftheta}.
\end{equation}
%
The parameters $\bftheta$ are updated using gradient descent by back-propagating the loss through the neural ODE solver using adjoint states $\bfy_i = \frac{\partial \calL}{\partial {\bfx_i}}$ \cite{chen2018neural}. We form an augmented state $\bfz_i = \prl{\bfx_i, \bfy_i, \frac{\partial \calL}{\partial \bftheta}}$ that satisfies $\dot{\bfz}_i = \bff_\bfz = \prl{\bff_i, -\bfy_i^\top \frac{\partial \bff_i}{\partial {\bfx_i}}, -\bfy_i^\top \frac{\partial \bff_i}{\partial \bftheta}}$. The gradients $\frac{\partial \calL}{\partial \bftheta}$ are obtained by solving a reverse-time ODE starting from $\bfz_i(rT) = \bar{\bfz}_i(rT)$:
%
\begin{equation}
\prl{\bfx_i(0), \bfy_i(0), \frac{\partial \calL}{\partial\bftheta}} = \mathsf{ODESolver}(\bfz_i(rT), \bff_z, rT).
\end{equation}
We refer the reader to \cite{chen2018neural} for more details.

% The port- Hamiltonian dynamics, specified by the learned port- Hamiltonian terms $\mathcal{F}_i$, is defined in the continuous-time, while the demonstration dataset $\bar{\mathcal{D}}$ is composed by discrete samples of the task. This is problematic because the learned control policies may not respect the physical restriction of the robots. We propose to learn $\bftheta$ through an ordinary differential equation solver~\cite{chen2018neural} to overcome this issue and preserve the physical laws of the robots.

% The training process is conducted by solving the following optimization problem, coined as LEMURS (\textbf{LE}arning distributed \textbf{MU}lti-\textbf{R}obot interaction\textbf{S}): 
% \begin{subequations}\label{eq:step2}
% \begin{alignat}{2}
% \min_{\bftheta} & \hbox{ }       \mathcal{L}({\mathcal{D}},\bar{\mathcal{D}}) \label{eq:step2cost}
% \\
% s.t. &  \hbox{ }{\mathbf{x}}_i^l(0) = \bar{\mathbf{x}}_i^l(0) \hbox{ } \forall i, l , \quad {\mathcal{F}}_i^l = \mathsf{SA}(\mathbf{X}^l_i,\bm{\theta}) \hbox{ } \forall i, l \label{eq:step2constraint1}
% \\
% & \hbox{ }{\mathbf{x}}^l_{i,1:K} = \mathsf{ODEsolver}(f_i, \pi_{\bftheta}, \bm{\theta}, \mathbf{x}^l(0), \mathcal{F}_i^l) \hbox{ } \forall i, l \label{eq:step2constraint3}
% \end{alignat}
% \end{subequations}


% The estimated states are calculated by an ordinary differential equation solver and the gradient of the loss function is back-propagated using adjoint methods~\cite{chen2018neural}. The parameters $\bftheta$ are updated using gradient descent. \TODO{Thai to add more details about neural ODE}

% Besides, note that the parameters $\bm{\theta}$ are shared across robots and the control policy does not depend on the number of robots in the team, so it is scalable to any robot team size. This is a significant difference with other approaches like multi-layer perceptrons and graph neural networks, where the size of the layers/filters depends on the number of robots, it is much more trickier to scale the policies.

\subsubsection{Deploying LEMURS}
\label{subsec:msg}
To deploy the control policy \eqref{eq:open_loop_intro_controller_ind_distributed}, we design a message $\mathbf{m}_{ij}(t)$, encoding information that robot $i$ needs from robot $j$ at time $t$ to calculate $[\mathbf{J}_{\bftheta}]_{ij}, [\mathbf{R}_{\bftheta}]_{ij}$, and $H_{\bftheta}^{(i)}$. When there is no communication among robots, i.e., $k=0$, no message $\mathbf{m}_{ij}(t)$ is needed. For $k > 1$, robot $i$ can calculate  $H_{\bftheta}^{(i)}$ from its own and neighbors' state $\bfx_j, j \in \calN_i^k$ as described in Sec. \ref{subsubsec:sa_architecture_JRH}. To calculate $\partial H_{\bftheta}/\partial \mathbf{x}_i = \sum_{j\in \calN_i}{\partial H^{(j)}_{\bftheta}/\partial \mathbf{x}_i}$, $[\mathbf{J}_{\bftheta}]_{ij}, [\mathbf{R}_{\bftheta}]_{ij}$, robot $i$ needs $\partial H^{(j)}_{\bftheta}/\partial \mathbf{x}_i$, ${\mathbf{Z}}_{ji}^{J}$ and ${\mathbf{Z}}_{ji}^{R}$ from neighbor $j$, which in turns depends on $k$-hop neighbors of robot $j$. In other words, these quantities depend on at most $2k$-hop neighbors of robot $i$. Finally, robot $i$ also needs $\partial H_{\bftheta}/\partial \mathbf{x}_j$ from neighbor $j$ to complete the control policy \eqref{eq:open_loop_intro_controller_ind_distributed}. 

In summary, each robot $i$ receives a message $\mathbf{m}_{ij} = [\mathbf{m}^{(1)}_{ij}, \mathbf{m}^{(2)}_{ij}, \mathbf{m}^{(3)}_{ij}]$ in $3$ communication rounds: 1) robot $i$ receives $\mathbf{m}^{(1)}_{ij} = \bfx_j$ $\forall j \in \calN_i^k$ and calculates ${\mathbf{Z}}_{ij}^{J}$, ${\mathbf{Z}}_{ij}^{R}$, $H_{\bftheta}^{(i)}$, and $\partial H^{(i)}_{\bftheta}/\partial \mathbf{x}_j$; 2) robot $i$ receives $\mathbf{m}^{(2)}_{ij} = \partial H^{(j)}_{\bftheta}/\partial \mathbf{x}_i, {\mathbf{Z}}_{ji}^{J}, {\mathbf{Z}}_{ij}^{R}$ $\forall j \in \calN_i^k$, and calculates $\partial H_{\bftheta}/\partial \mathbf{x}_i$, $[\mathbf{J}_{\bftheta}]_{ij}, [\mathbf{R}_{\bftheta}]_{ij}$; and 3) each robot $i$ receives $\mathbf{m}^{(3)}_{ij} = \partial H_{\bftheta}/\partial \mathbf{x}_j$ $\forall j \in \calN_i^k$ and calculates the control input $\bfu_i$.
% The formulation of LEMURS allows to consider as many hops as desired. For a fully distributed setup, $k=0, 1$: the former implies that robots do not communicate, which restricts the class of tasks that can be learned; the latter includes information form neighbors. Notice that, to calculate $\mathbf{u}_i$ in the deployment time, robot $i$ needs the information of $(k+1)$-hop neighbors due to $\partial H_{\bftheta}(\mathbf{x}) / \partial \mathbf{x}_j$. To solve this, one option is that robots exchange information in three communication rounds: 1) robot $i$ receives the messages $\mathbf{m}_{ij} = \{\bfx_j\}$  and computes $\frac{\partial H_{\bftheta}^{(i,k)}}{\partial \bfx_j}$; 2) robot $i$ receives the messages $\mathbf{m}_{ij} = \{\frac{\partial H_{\bftheta}^{(j,k)}}{\partial \bfx_i}\}$ and computes $\frac{\partial H}{\partial \bfx_i} = \sum_{j \in \mathcal{N}_i^k \cup \{i\}} \frac{\partial H^{(j,k)}}{\partial \bfx_i}$; 3) robot $i$ receives the messages $\mathbf{m}_{ij} = \{\frac{\partial H_{\bftheta}(\bfx)}{\partial \bfx_j}\}$. This is only critical for an efficient distributed deployment. 
We assume negligible delays between communication rounds. If the delay is large, Wang et al. ~\cite{wang2022darl1n} suggest to learn a function that predicts quantities such as $\partial H_{\bftheta}(\mathbf{x}) / \partial \mathbf{x}_j$, ${\mathbf{Z}}_{ji}^{J}$, ${\mathbf{Z}}_{ji}^{R}$, leading to one communication round. We leave this for future work. If the Hamiltonian changes slowly over sampling interval $T$, at time $t = rT$, robot $i$ can use its previous neighbor states $\bfx_j ((r-1)T)$ to approximate $\mathbf{m}^{(2)}_{ij}(rT)$ and $\mathbf{m}^{(3)}_{ij}(rT)$. 

% Besides, the port-Hamiltonian constraints are preserved, so the learned control policies guarantee that the robot trajectories do not diverge. This is a significant feature of our proposal in contrast to the state-of-the-art. 

% The convergence to the fulfillment of the task depends on a good training, such that LEMURS uncovers what the equilibrium of the task $\mathbf{x}^*$ is and $\arg \min_\mathbf{x} H(\mathbf{x}) = \mathbf{x}^*$\NA{I removed the mentioning of equilibria earlier so we do not need to mention that here either.}. 


\begin{example}\label{example:flockingsolution}
In the flocking of Examples~\ref{example:flocking_controller}-\ref{example:portHamiltonian}, LEMURS can be directly applied to learn $\mathbf{D}_{\bftheta}(\mathbf{p})$ and ${U}_{\bftheta}(\mathbf{p})$. Another option is to learn $\mathbf{J}_{\bftheta}(\mathbf{x}), \mathbf{R}_{\bftheta}(\mathbf{x})$ and ${H}_{\bftheta}(\mathbf{x})$, obtaining extra degrees of freedom for the control policy.
\end{example}

==> 03_ProposedSolution_unused.tex <==
In this section, we present a port-Hamiltonian formulation of the multi-robot system, modeling unknown robot interactions as energy dissipation and exchange among the robots, and an energy-based distributed control design with stability guarantees (Sec. \ref{subsec:portHamiltonian}). Given demonstrated state trajectories of a task, the Hamiltonian structure allows us to learn robot interactions and design a stable distributed control policy from demonstration, using self-attention techniques and neural ordinary differential equation networks (Sec. \ref{subsec:LEMURS}). In the following, we omit the time-dependency in $\mathbf{x}$ and $\mathbf{u}$ for readability. 

%In this Section the technical approach to solve problem~\eqref{eq:prob_def} is presented. In Subsection~\ref{subsec:portHamiltonian} we move from the individual robot to the system dynamics by means of port-Hamiltonian mechanics, showing the convenience of this formulation in terms of stability, scalability and distributed behavior. In Subsection~\ref{subsec:LEMURS} we return to the robot dynamics level to present the learning proposal to solve~\eqref{eq:prob_def}.  

\subsection{Port-Hamiltonian Formulation of Multi-Robot Systems}\label{subsec:portHamiltonian}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As a physical system, the individual robot dynamics \eqref{eq:known_dynamics} formulated in Section~\ref{sec:prosta} satisfy port-Hamiltonian mechanics \cite{van2014port} for $i = 1, \ldots, n$ with the state $\bfx_i = [\frakq_i, \frakp_i]~\in~\bbR^{n_x}$ consisting of generalized coordinates $\frakq_i \in \bbR^{n_s}$ and generalized momentum $\frakp_i \in \bbR^{n_s}$ and $n_x = 2n_s$:
\begin{equation}\label{eq:open_loop_intro_individual}
% \begin{aligned}
%         \begin{bmatrix} \dot{\frakq}_i \\ \dot{\frakp_i} \end{bmatrix} &= \left(\mathbf{J}_s^{(i)}(\mathbf{x}_i) - \begin{bmatrix}
%         \mathbf{0} & \mathbf{0} \\ \mathbf{0} & \mathbf{R}_s^{(i)}(\mathbf{x}_i)
%         \end{bmatrix}\right) \begin{bmatrix} \frac{\partial {\calH}_s^{(i)}(\mathbf{x}_i)}{\partial\frakq_i} \\ \frac{\partial {\calH}_s^{(i)}(\mathbf{x}_i)}{\partial\frakp_i} \end{bmatrix} \\
%         & \qquad \qquad\qquad \qquad  + \begin{bmatrix} \mathbf{0} \\ \mathbf{F}_s^{(i)}(\mathbf{x}_i) \end{bmatrix}\mathbf{u}_i,
% \end{aligned}
    \scaleMathLine{\begin{bmatrix} \dot{\frakq}_i \\ \dot{\frakp}_i \end{bmatrix} = \left(\calJ_s^{(i)}(\mathbf{x}_i) - \calR_s^{(i)}(\bfx_i) \right) \begin{bmatrix}\frac{\partial {\calH}_s^{(i)}(\mathbf{x}_i)}{\partial\frakq_i} \\ \frac{\partial {\calH}_s^{(i)}(\mathbf{x}_i)}{\partial\frakp_i} \end{bmatrix} + \calF_s^{(i)}(\mathbf{x}_i)\mathbf{u}_i,}
\end{equation}
where the skew-symmetric interconnection matrix $$\calJ_s^{(i)}(\bfx_i) = \begin{bmatrix}
\bfJ_{s\frakq\frakq}^{(i)}(\bfx_i) & \bfJ_{s\frakq\frakp}^{(i)}(\bfx_i) \\ \bfJ_{s\frakp\frakq}^{(i)}(\bfx_i)  & \bfJ_{s\frakp\frakp}^{(i)}(\bfx_i)\end{bmatrix}$$
represents energy exchange \emph{within a robot}, e.g., between its kinetic and potential energy, the dissipation matrix $\calR_s^{(i)}(\bfx_i) = \begin{bmatrix}
        \mathbf{0} & \mathbf{0} \\ \mathbf{0} & \mathbf{R}_s^{(i)}(\mathbf{x}_i)
        \end{bmatrix}$ \footnote{This applies to robot dynamics. It might not be true for other systems like electric or chemical systems.} represents energy dissipation, e.g., from friction, the total energy is ${\calH}_s^{(i)}(\mathbf{x}_i)$, and the input gain is $\calF_s^{(i)}(\bfx_i)$. 

The multi-robot system with joint state $\bfx~=~[\frakq, \frakp]~=~[\frakq_1, \ldots, \frakq_n, \frakp_1, \ldots, \frakp_n]$, consisting of generalized coordinates $\frakq$ and momentum $\frakp$ of $n$ robots, also satisfies the (port)-Hamiltonian formulation:
\begin{equation}\label{eq:open_loop_intro}
\begin{bmatrix} \dot{\frakq} \\ \dot{\frakp} \end{bmatrix} = \left(\calJ_s(\mathbf{x}) - \calR_s(\bfx)\right) \begin{bmatrix} \frac{\partial {\calH}_s(\mathbf{x})}{\partial\frakq} \\ \frac{\partial {\calH}_s(\mathbf{x})}{\partial\frakp} \end{bmatrix} + \calF_s(\mathbf{x})\mathbf{u},
\end{equation}
where the skew-symmetric interconnection matrix $$\calJ_s = \begin{bmatrix}
\bfJ_{s\frakq\frakq}(\bfx) & \bfJ_{s\frakq\frakp}(\bfx) \\ \bfJ_{s\frakp\frakq}(\bfx)  & \bfJ_{s\frakp\frakp}(\bfx)\end{bmatrix},$$ the positive semidefinite dissipation matrix $\calR_s = \begin{bmatrix}
        \mathbf{0} & \mathbf{0} \\ \mathbf{0} & \mathbf{R}_s(\mathbf{x})
        \end{bmatrix}$ and the input gain $\calF_s^{(i)}$ have the following block-diagonal form:
\begin{equation}\label{eq:block_diag_structureo}
\begin{aligned}
    \bfJ_{sk}(\bfx) &= \diag\left(\bfJ_{sk}^{(1)}(\bfx_1), \ldots, \bfJ_{sk}^{(n)}(\bfx_n) \right), k = \frakq\frakq, \frakq\frakp, \frakp\frakq, \frakp\frakp, \\
    \bfR_s(\bfx) &= \diag\left(\bfR_s^{(1)}(\bfx_1), \ldots, \bfR_s^{(n)}(\bfx_n) \right), \\
    \calF_s(\bfx) &= \diag\left(\calF_s^{(1)}(\bfx_1), \ldots, \calF_s^{(n)}(\bfx_n) \right), \\
\end{aligned}
\end{equation}
and with $\calH_s(\bfx) = \sum_{i=1}^n \calH_s^{(i)}(\bfx_i)$ the total energy.

Given a desired state $\bfx^*$, the original Hamiltonian system \eqref{eq:open_loop_intro} without any control input does not converge to $\bfx^*$ as the total energy $\calH_s(\bfx)$ is not minimized at $\bfx^*$. To drive the system to $\bfx^*$, we employ the interconnection
and damping assignment passivity-based control (IDA-PBC) approach \cite{van2014port}, which injects additional energy to the system through the control input $\bfu$ so that the system has a desired total energy $\calH(\bfx)$ with a minimizer $\bfx^*$. The closed-loop multi-robot system, i.e., with a joint control policy $\bfu = \bfpi(\bfx)$, satisfies a desired Hamiltonian dynamics:
\begin{equation}\label{eq:closed_loop_intro}
        \dot{\mathbf{x}} = \left( \calJ(\mathbf{x})   -  \calR(\mathbf{x})\right)
\frac{\partial {\calH}(\mathbf{x})}{\partial\mathbf{x}}, 
\end{equation}
where $\bfJ(\bfx) = \begin{bmatrix}
\bfJ_{\frakq\frakq}(\bfx) & \bfJ_{\frakq\frakp}(\bfx) \\ \bfJ_{\frakp\frakq}(\bfx)  & \bfJ_{\frakp\frakp}(\bfx)\end{bmatrix}$ is the desired skew-symmetric interconnection matrix and $\calR(\bfx) = \begin{bmatrix}
        \mathbf{0} & \mathbf{0} \\ \mathbf{0} & \mathbf{R}(\mathbf{x})
        \end{bmatrix}$ is the desired positive semidefinite dissipation matrix. This desired Hamiltonian dynamics represent the task we want to replicate. 
By matching \eqref{eq:open_loop_intro} and \eqref{eq:closed_loop_intro}, we can derive the control input as follows:
\begin{equation}\label{eq:open_loop_intro_controller}
\begin{aligned}
\mathbf{u} &= \calF_s^{\dagger}(\mathbf{x})
\left(\prl{\calJ(\bfx) - \calR(\mathbf{x})}\frac{\partial {\calH}(\mathbf{x})}{\partial\mathbf{x}} \right. 
\\
& \qquad \quad \kern 0.2cm- \left.\prl{\calJ_s(\bfx) - \calR_s(\mathbf{x})}\frac{\partial {\calH}_s(\mathbf{x})}{\partial\mathbf{x}} \right),
\end{aligned}
\end{equation}
where $\calF_s^{\dagger}(\mathbf{x}) = \left(\calF_s^{T}(\bfx)\calF_s(\bfx)\right)^{-1}\calF_s^{T}(\bfx)$ is the pseudo-inverse of $\calF_s(\mathbf{x})$. The control $\bfu$ exists as long as the following matching conditions are satisfied:
\begin{equation}\label{eq:matching_condition}
\begin{aligned}
\calF_s^{\perp}(\mathbf{x})
& \left(\prl{\calJ(\bfx) - \calR(\mathbf{x})}\frac{\partial {\calH}(\mathbf{x})}{\partial\mathbf{x}} \right. 
\\
& \qquad \quad \kern 0.2cm- \left.\prl{\calJ_s(\bfx) - \calR_s(\mathbf{x})}\frac{\partial {\calH}_s(\mathbf{x})}{\partial\mathbf{x}} \right) = 0,
\end{aligned}
\end{equation}
where $\calF_s^{\perp}(\mathbf{x})$ is the maximal-rank left annihilator of $\calF_s(\mathbf{x})$, i.e. $\calF_s^{\perp}(\mathbf{x})\calF_s(\mathbf{x}) = 0$. 
% As the control input $\bfu_i$ only affects the robot $i$, the input gain matrix $\calF_s(\mathbf{x})$ is block-diagonal: 
% \begin{equation}
%     \calF_s(\bfx) = \diag\prl
% {\calF_s^{(1)}(\bfx_1), \ldots, \calF_s^{(n)}(\bfx_n)},
% \end{equation}
% where $\calF_s^{(i)}(\bfx_i)$ is the input gain matrix for robot $i$. This allows each robot $i$ to evaluate the matching conditions and calculate its control input $\bfu_i$ locally using \eqref{eq:open_loop_intro_controller}. 

Assuming the matching conditions are satisfied, the closed-loop system \eqref{eq:closed_loop_intro} is stable around $\bfx^*$ in the sense of Lyapunov \cite{van2014port} with $\partial {\calH}(\bfx)/\partial \bfx = \mathbf{0}$ at $\bfx = \bfx^*$. In the control policy \eqref{eq:open_loop_intro_controller}, $\calJ_s(\bfx)$, $\calR_s(\bfx)$, $\calF_s(\bfx)$ and $\calH_s(\bfx)$ are known, representing the robot individual dynamics. Meanwhile, the desired matrices $\calJ(\bfx)$ and $\calR(\bfx)$ represent the robot interactions by exchanging and dissipating energy according to the robot interaction graph $\mathcal{G}$ in Sec. \ref{sec:prosta}, so that the closed-loop system converges to $\bfx^*$ and fulfills the task.

Given demonstrated state trajectories, the Hamiltonian structure and the IDA-PBC control design \eqref{eq:open_loop_intro_controller} reduce the problem of learning the control policy in \eqref{eq:prob_def} to finding a desired skew-symmetric interconnection matrix $\calJ(\mathbf{x})$, a desired positive semidefinite dissipation matrix $\bfR(\mathbf{x}) \succeq \mathbf{0}$ and a desired Hamiltonian ${\calH}(\mathbf{x}) \geq 0$ to minimize the loss function \eqref{eq:loss_function}. We derive the conditions such that the control policy \eqref{eq:open_loop_intro_controller} is distributed, i.e., each robot calculates its own control input $\bfu_i$ from its own state $\bfx_i$ and its neighbors' states $\bfx_j, j\in\calN_i$.

We consider the desired total energy $\calH(\bfx)$ of the form:
\begin{equation}
    \calH(\bfx) = \bfx^\top \bfM(\bfq) \bfx + \calU(\bfq),
\end{equation}
where the first term represents the desired interaction 



Let $[\mathbf{J}(\mathbf{x})]_{i}$ and $[\mathbf{R}(\mathbf{x})]_{i}$ denote the $i$th $n_x \times n n_x$ row blocks and $[\mathbf{J}(\mathbf{x})]_{ij}$ and $[\mathbf{R}(\mathbf{x})]_{ij}$ denote the $n_x \times n_x$ blocks with index $(i,j)$. To make the controller distributed, robot $i$ must be able to calculate $[\mathbf{J}(\mathbf{x})]_{i}$,  $[\mathbf{R}(\mathbf{x})]_{i}$, and $\partial H/\partial \bfx_i$ only from $\bfx_i$ and $\bfx_j, j \in \calN_i$. In the following, we derive the general conditions that restrict the port-Hamiltonian systems to be distributed.

First, the state in port-Hamiltonian systems is composed by the generalized coordinates $\mathbf{q}$ and momenta $\mathbf{p}$, such that $\mathbf{x} = [\mathbf{q}^T, \mathbf{p}^T]^T$. This holds for every port-Hamiltonian system. Then, the Hamiltonian energy function is described by means of $\mathbf{q}$ and $\mathbf{p}$ as follows:
% \begin{equation}\label{eq:Hq}
%     \begin{aligned}
%         {\calH}(\mathbf{q}, \mathbf{p}) =& [\mathbf{q}^T, \mathbf{p}^T] \mathbf{M}(\mathbf{q})[\mathbf{q}^T, \mathbf{p}^T]^T + {P}(\mathbf{p}) =
%         \\&
%         [\mathbf{q}^T, \mathbf{p}^T] 
%         \begin{pmatrix}
%         \mathbf{M}_{\mathbf{q}\mathbf{q}} & \mathbf{M}_{\mathbf{q}\mathbf{p}}
%         \\
%         \mathbf{M}_{\mathbf{p}\mathbf{q}} & \mathbf{M}_{\mathbf{p}\mathbf{p}}
%         \end{pmatrix}
%         [\mathbf{q}^T, \mathbf{p}^T]^T + {P}(\mathbf{q})
%     \end{aligned}
% \end{equation}
\begin{equation}\label{eq:Hq}
    \begin{aligned}
        {\calH}(\mathbf{q}, \mathbf{p}) =& [\mathbf{q}^T, \mathbf{p}^T] \mathbf{M}(\mathbf{q})[\mathbf{q}^T, \mathbf{p}^T]^T + {P}(\mathbf{p}) =
        \\&
        [\mathbf{q}^T, \mathbf{p}^T] 
        \begin{pmatrix}
        \mathbf{M}_{\mathbf{q}\mathbf{q}} & \mathbf{M}_{\mathbf{q}\mathbf{p}}
        \\
        \mathbf{M}_{\mathbf{p}\mathbf{q}} & \mathbf{M}_{\mathbf{p}\mathbf{p}}
        \end{pmatrix}
        [\mathbf{q}^T, \mathbf{p}^T]^T + {P}(\mathbf{q})
    \end{aligned}
\end{equation}
where the first term represents the kinetic energy and the second term is the potential energy. Restriction $\mathbf{M}(\mathbf{p}) \succeq \mathbf{0}$ holds. Again, this holds for every port-Hamiltonian systems, so generality is preserved. Therefore, Eq.~\eqref{eq:closed_loop_intro} reads 
\begin{equation}\label{eq:closed_loop_ext}
        \kern -0.3cm \begin{pmatrix}
        \dot{\mathbf{q}} \\ \dot{\mathbf{p}}
        \end{pmatrix} 
        = \left( 
        \begin{pmatrix}
        \mathbf{J}_{\mathbf{q}\mathbf{q}} & \mathbf{J}_{\mathbf{q}\mathbf{p}}
        \\
        \mathbf{J}_{\mathbf{p}\mathbf{q}} & \mathbf{J}_{\mathbf{p}\mathbf{p}}
        \end{pmatrix} -
        \begin{pmatrix}
        \mathbf{R}_{\mathbf{q}\mathbf{q}} & \mathbf{R}_{\mathbf{q}\mathbf{p}}
        \\
        \mathbf{R}_{\mathbf{p}\mathbf{q}} & \mathbf{R}_{\mathbf{p}\mathbf{p}}
        \end{pmatrix}\right)
        \begin{pmatrix}
        \frac{\partial {\calH}}{\partial\mathbf{q}} \\ \frac{\partial {\calH}}{\partial\mathbf{p}}
        \end{pmatrix}.
\end{equation}
Besides, let $[\mathbf{J}_{\mathbf{k}\mathbf{\calH}}]_{i}$, $[\mathbf{R}_{\mathbf{k}\mathbf{\calH}}]_{i}$, $[\mathbf{M}_{\mathbf{k}\mathbf{\calH}}]_{i}$ denote the $i$th $n_x/2 \times n n_x/2$ row blocks and $[\mathbf{J}_{\mathbf{k}\mathbf{\calH}}]_{ij}$, $[\mathbf{R}_{\mathbf{k}\mathbf{\calH}}]_{ij}$,
$[\mathbf{M}_{\mathbf{k}\mathbf{\calH}}]_{ij}$ denote the $n_x/2 \times n_x/2$ blocks with index $k,h = \{\mathbf{q}, \mathbf{p}\}$; and let $\frac{\partial {\calH}}{\partial\mathbf{q}_{i}}$, $\frac{\partial {\calH}}{\partial\mathbf{p}_{i}}$ $\forall i \in \mathcal{V}$.
From the definition of the Hamiltonian in~\eqref{eq:Hq}, 
\begin{align}\label{eq:partials_q}
    &\frac{\partial {\calH}}{\partial\mathbf{p}} = \mathbf{M}_{\mathbf{q}\mathbf{p}}\mathbf{q} + \mathbf{M}^T_{\mathbf{p}\mathbf{q}}\mathbf{q} + \mathbf{M}^T_{\mathbf{p}\mathbf{p}}\mathbf{p} + \mathbf{M}_{\mathbf{p}\mathbf{p}}\mathbf{p},
    \\
    &\begin{aligned}\label{eq:partials_p}
    \frac{\partial {\calH}}{\partial\mathbf{q}} =&\mathbf{M}_{\mathbf{q}\mathbf{q}}\mathbf{q} + \mathbf{M}_{\mathbf{q}\mathbf{p}}\mathbf{q} + \mathbf{M}_{\mathbf{p}\mathbf{q}}\mathbf{q} + \mathbf{M}_{\mathbf{p}\mathbf{p}}\mathbf{p} + 
    \\&
    [\mathbf{q}^T, \mathbf{p}^T] \frac{\partial \mathbf{M}}{\partial\mathbf{q}}[\mathbf{q}^T, \mathbf{p}^T]^T +  \frac{\partial {P}}{\partial\mathbf{p}}.
    \end{aligned}
\end{align}
BY inspection, the partial of the Hamiltonian with respect to the momentum can be computed in a distributed way if $\mathbf{M}$ is compatible with the graph, so it can be computed in a distributed way; meanwhile, due to $\frac{\partial \mathbf{M}}{\partial\mathbf{q}}$ and $\frac{\partial P}{\partial\mathbf{q}}$, the partial of the Hamiltonian with respect to the generalized coordinated couples the local states of all the robots. Therefore, for a fully distributed computation, the following requirements are needed:
\begin{equation} 
\label{eq:JRH_conditions}
\begin{aligned}
        \frac{\partial}{\partial \bfx_j} \frac{\partial H}{\partial \bfx_i} &= 0, \forall j \notin \calN_i,
        \\
        \mathbf{J}_{\mathbf{q}\mathbf{q}} &= \mathbf{J}_{\mathbf{p}\mathbf{p}} = \mathbf{0}, 
        \\
        [\mathbf{J}_{\mathbf{p}\mathbf{q}}]_{ij} &=[\mathbf{J}_{\mathbf{q}\mathbf{p}}]_{ij} =\mathbf{0}, \forall j \neq i, 
        \\
        \mathbf{R}_{\mathbf{q}\mathbf{q}} &= \mathbf{R}_{\mathbf{p}\mathbf{q}} =  \mathbf{R}_{\mathbf{q}\mathbf{p}} = \mathbf{0}, 
        \\
        [\mathbf{R}_{\mathbf{p}\mathbf{p}}]_{ij} &= \mathbf{0}, \forall j \neq \calN_i.
        \\
        [\mathbf{M}_{\mathbf{k}\mathbf{\calH}}]_{ij} &= \mathbf{0}, \forall j \neq \calN_i \text{ and } \mathbf{k}, \mathbf{\calH} \in \{\mathbf{q}, \mathbf{p}\}
\end{aligned}
\end{equation}
Thus, the IDA-PBC yields to the following individual control policy $\pi(\;)$ on Eq.~\eqref{eq:general_controller}:
\begin{equation}\label{eq:open_loop_intro_controller_ind}
\begin{aligned}
\kern -5pt \mathbf{u}_i &= \calF_s^{\dagger}(\mathbf{x}_i)
\left(-\left(\mathbf{J}_s^{(i)}(\mathbf{x}_i) - \mathbf{R}_s^{(i)}(\mathbf{x}_i)\right)\frac{\partial {\calH}_s^{(i)}(\mathbf{x})}{\partial\mathbf{x}_i} + \right. 
\\
& \left.
\begin{pmatrix}
[\mathbf{J}_{\mathbf{p}\mathbf{q}}]_{ii} \frac{\partial \calH(\mathbf{x})}{\partial \mathbf{p}_i}
\\
[\mathbf{J}_{\mathbf{q}\mathbf{p}}]_{ii} \frac{\partial \calH(\mathbf{x})}{\partial \mathbf{q}_i} + \sum_{j \in \mathcal{N}_i \cup \{i\}}[\mathbf{R}_{\mathbf{p}\mathbf{p}}]_{ij}\frac{\partial \calH(\mathbf{x})}{\partial \mathbf{p}_j} 
\end{pmatrix}
\right),
\end{aligned}
\end{equation}
% \begin{equation} \label{eq:JRH_conditions}
%     \begin{aligned}
%         \frac{\partial}{\partial \bfx_j}\prl{\frac{\partial H}{\partial \bfx_i}} &=& \mathbf{0}, \quad\forall j \notin \calN_i \\
%         [\mathbf{J}(\mathbf{x})]_{ij} & = & \mathbf{0}, \quad\forall j \notin \calN_i \\
%         [\mathbf{R}(\mathbf{x})]_{ij} & = & \mathbf{0}, \quad\forall j \notin \calN_i.
%     \end{aligned}
% \end{equation}
The takeaway of Sec. \ref{subsec:portHamiltonian} is that a distributed structure can be derived for general port-Hamiltonian systems. The (port-Hamiltonian) and distributed requirements for $\mathbf{J}(\mathbf{x})$, $\mathbf{R}(\mathbf{x}) \succeq \mathbf{0}$ and ${H}(\mathbf{x})$ are used, in Sec. \ref{subsec:LEMURS}, to design our model of robot interaction and control, inheriting stability guarantees from the IDA-PBC approach while staying distributed.

%In other words, by using the port- Hamiltonian formulation, we transform the original problem, an unstructured learning problem within a large class of control policies, to a structured learning problem within a tighter class of stable and distributed control policies by construction. 
%In the next Subsection we propose a solution to learn $\mathbf{R}(\mathbf{x}), \mathbf{J}(\mathbf{x})$ and ${H}(\mathbf{x})$ such that they respect both the port-Hamiltonian, stability and distributed constraints.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The dynamics formulated in Section~\ref{sec:prosta} is completely unstructured, for there is no particular restriction in the class of policies that solve problem~\eqref{eq:prob_def}. This hinders the learning problem because the control policy not only has to accomplish the task, but also it must guarantee a stable and distributed behavior of the multi-robot team in order to succeed in general settings. We propose a port-Hamiltonian~\cite{shaft2004port} description of the system to exploit universal physical constraints over networked systems and guarantee a stable and distributed control policy by construction.

% The port-Hamiltonian description of a general interconnected system is 
% \begin{equation}\label{eq:closed_loop_intro}
%         \dot{\mathbf{x}} = \left( \mathbf{J}(\mathbf{x})   -   \mathbf{R}(\mathbf{x})\right)
% \frac{\partial {H}(\mathbf{x})}{\partial\mathbf{x}}, 
% \end{equation}
% where ${H}(\mathbf{x}) \geq 0$ is the \textbf{Hamiltonian} (i.e., total energy) of the system, $\mathbf{J}(\mathbf{x})$ is a skew-symmetric \textbf{interconnection matrix} ($\mathbf{J}(\mathbf{x}) + \mathbf{J}^T(\mathbf{x}) = \mathbf{0}$), and $\mathbf{R}(\mathbf{x})$ is a positive semidefinite \textbf{dissipation matrix} ($\mathbf{R}(\mathbf{x}) \succeq \mathbf{0}$). In terms of the multi-robot system,  $\mathbf{J}(\mathbf{x})$ and $\mathbf{R}(\mathbf{x})$ model how robots interact (by exchanging and dissipating energy) so that the system converges to a minimum-energy equilibrium point that corresponds to the fulfillment of the task. Nevertheless, Eq.~\eqref{eq:closed_loop_intro} is the closed-loop dynamics of the system. In the absence of a known controller, the multi-robot system is described by open-loop input-state-output port-Hamiltonian dynamics 
% \begin{equation}\label{eq:open_loop_intro}
%         \dot{\mathbf{x}} = \left(\mathbf{J}_s(\mathbf{x}) - \mathbf{R}_s(\mathbf{x})\right)\frac{\partial {H}_s(\mathbf{x})}{\partial\mathbf{x}} + \mathbf{F}_s^T(\mathbf{x})\mathbf{u}.
% \end{equation}
% Here, ${H}_s(\mathbf{x}), \mathbf{J}_s(\mathbf{x}), \mathbf{R}_s(\mathbf{x})$ are the open-loop Hamiltonian, interconnection matrix and dissipation matrix respectively, and $\mathbf{F}_s(\mathbf{x})$ is an input matrix. The aim of the control policy is to obtain Eq.~\eqref{eq:closed_loop_intro} from Eq.~\eqref{eq:open_loop_intro}. Interestingly, the port-Hamiltonian description allows to define the controller as another energy system with a port-Hamiltonian description~\cite{yuksel2014reshaping}, since the interconnection of two port-Hamiltonian systems is another port-Hamiltonian system~\cite{shaft2004port}. In particular, the interconnection
% and damping assignment passivity-based controller (IDA-PBC) 
% \begin{equation}\label{eq:open_loop_intro_controller}
% \begin{aligned}
% \mathbf{u} =& \mathbf{F}_s^{\dagger}(\mathbf{x})
% \left( \left(\mathbf{J}(\mathbf{x}) - \mathbf{R}(\mathbf{x})\right)\frac{\partial {H}(\mathbf{x})}{\partial\mathbf{x}} \right.
% \\
% & 
% -
% \left.\left(\mathbf{J}_s(\mathbf{x}) - \mathbf{R}_s(\mathbf{x})\right)\frac{\partial {H}_s(\mathbf{x})}{\partial\mathbf{x}} \right)
% \end{aligned}
% \end{equation}
% yields to the desired closed-loop behavior~\cite{van2014port}. Notice that ${H}(\mathbf{x}) = {H}_s(\mathbf{x}) + {H}_u(\mathbf{x})$, i.e.,  the total energy of the system is the sum of the energy of the open-loop dynamics and the energy injected by the controller. \NEWTD{The control $\bfu$ exists as long as the following matching conditions are satisfied:
% \begin{equation}\label{eq:matching_condition}
% \begin{aligned}
% \mathbf{F}_s^{\perp}(\mathbf{x})
% & \left( \left(\mathbf{J}(\mathbf{x}) - \mathbf{R}(\mathbf{x})\right)\frac{\partial {H}(\mathbf{x})}{\partial\mathbf{x}} \right.
% \\
% &-
% \left.\left(\mathbf{J}_s(\mathbf{x}) - \mathbf{R}_s(\mathbf{x})\right)\frac{\partial {H}_s(\mathbf{x})}{\partial\mathbf{x}} \right) = 0,
% \end{aligned}
% \end{equation}
% where $\mathbf{F}_s^{\perp}(\mathbf{x})$ is the maximal-rank left annihilator of $\mathbf{F}_s(\mathbf{x})$, i.e. $\mathbf{F}_s^{\perp}(\mathbf{x})\mathbf{F}_s(\mathbf{x}) = 0$.
% As the control input $\bfu_i$ only affects the robot $i$, the input gain matrix $\mathbf{F}_s(\mathbf{x})$ is block-diagonal: 
% \begin{equation}
%     \bfF_s(\bfx) = \diag\prl
% {\bfF_s^{(1)}(\bfx_1), \ldots, \bfF_s^{(n)}(\bfx_n)},
% \end{equation}
% where $\bfF_s^{(i)}(\bfx_i)$ is the input gain matrix for robot $i$ \TODO{Update notation if the input gain for each robot $i$ is defined in the Problem Statement}. This allows each robot $i$ to evaluate the matching conditions and calculate its control input $\bfu_i$ locally using \eqref{eq:open_loop_intro_controller}. 

% Let $\bfx^*$ be an equilibrium where the Hamiltonian $\calH(\bfx)$ achieves its minimum. Assuming the matching conditions are satisfied, e.g. when each robot is fully-actuated, i.e. $\bfF_s(\bfx)$ is full-rank, the close-loop system \eqref{eq:closed_loop_intro} is stable around $\bfx^*$ in the sense of Lyapunov with $\partial {H}(\bfx^*)/ \partial \bfx^*  = \mathbf{0}$ and $\calH(\bfx^*) = 0$ \cite{van2014port}.

% \NA{This is hard to follow for someone who is not familiar with port-Hamiltonian systems. What are the blocks of $\mathbf{F}_s$ and how do they relate to the individual agent dynamics? It might be more intuitive to start the construction from an individual level, talk about the port-Hamiltonian description of the open-loop system and finally design the controller to achieve a desired closed-loop system.}. 
%}
% Besides, we assume that either $\mathbf{F}_s(\mathbf{x})$ is a block-diagonal matrix and $\mathbf{F}_s^{\dagger}(\mathbf{x})$ exists, so it can be computed locally by each robot; or each robot can compute locally the matching conditions that guarantee the existence of $\mathbf{F}_s^{\dagger}(\mathbf{x})$~\cite{yuksel2014reshaping,duong2021hamiltonian}\NA{This is hard to follow for someone who is not familiar with port-Hamiltonian systems. What are the blocks of $\mathbf{F}_s$ and how do they relate to the individual agent dynamics? It might be more intuitive to start the construction from an individual level, talk about the port-Hamiltonian description of the open-loop system and finally design the controller to achieve a desired closed-loop system.}. 


% Observe that, now, the problem of learning the control policy is reduced to finding $\mathbf{J}(\mathbf{x}), \mathbf{R}(\mathbf{x})$ and ${H}(\mathbf{x})$ that solve Eq.~\eqref{eq:prob_def}. The port-Hamiltonian constraints $\mathbf{J}(\mathbf{x}) + \mathbf{J}^T(\mathbf{x})  = \mathbf{0}$,  $\mathbf{R}(\mathbf{x})  \succeq \mathbf{0}$ and ${H}(\mathbf{x})  \geq \mathbf{0}$ must be guaranteed and the robots must be able to compute  $[{H}(\mathbf{x})]_i$ and $[\mathbf{R}(\mathbf{x})]_{ij}, [\mathbf{J}(\mathbf{x})]_{ij}$ $\forall j \in \mathcal{N}_i$ from local information only. By doing so the stability and distributed properties are ensured. Regarding stability, the next result proves that the control policy in Eq.~\eqref{eq:open_loop_intro_controller} guarantees the stability of the closed-loop system under the constraints imposed by the port-Hamiltonian description of the system.

% \NA{The statement of Proposition 1 should include the matching conditions. It is not true that stability can be achieved in general. I am also not sure if Propostion 1 is needed at all since it does not say anything different with respect to what is already known in passivity-based control for (port) Hamiltonian systems. We can state any of the desired properties in the text instead of highlighting as a proposition because the reviewers (at least if I were one) might question the novelty and correctness of Proposition 1.} 

% \begin{proposition}\label{prop:stability}
% The control policy in Eq.~\eqref{eq:open_loop_intro_controller} guarantees the stability of the system in Eq.~\eqref{eq:open_loop_intro} in the Lyapunov sense if $\mathbf{J}(\mathbf{x}) + \mathbf{J}^T(\mathbf{x})  = \mathbf{0}$,  $\mathbf{R}(\mathbf{x})  \succeq \mathbf{0}$ and ${H}(\mathbf{x})  \geq {0}$, and $\partial {H}(\mathbf{x})/ \partial \mathbf{x}  = \mathbf{0}$ 
% % \TD{I am a bit unclear why $\mathbf{J}(\mathbf{x}) = \mathbf{R}(\mathbf{x})  = \mathbf{0}$ at an equilibrium? It does not seem to be satisfied by the closed loop dynamics in Eq. \eqref{eq:closed_loop_Ham}} \ES{that was because the initial architecture couldn't ensure $dH/dx=0$ at equilibrium, so the condition was required to obtain $\dot{V} = 0$ at equilibrium. But the modification of the H architecture now implies $dH/dx = 0$ at equilibrium. Therefore, I have modified the proposition accordingly. Thanks!}
% and ${H}(\mathbf{x}) = {0}$ at equilibrium.
% \end{proposition}
% \begin{proof}
% The closed-loop dynamics in Eq.~\eqref{eq:closed_loop_intro} is obtained by substitution of the control policy of Eq.~\eqref{eq:open_loop_intro_controller} in the open-loop dynamics of Eq.~\eqref{eq:open_loop_intro}. The stability of the closed-loop system is therefore analyzed from Eq.~\eqref{eq:closed_loop_intro}. Without loss of generality, consider $\mathbf{x} = \mathbf{0}$ the desired equilibrium point and $\calH(\mathbf{x})$ the Lyapunov function candidate such that $\calH(\mathbf{x}) = 0$ if $\mathbf{x} = \mathbf{0}$ and $\calH(\mathbf{x}) > 0$ otherwise. The time derivative is
% \begin{equation}\label{eq:Vdot}
% \begin{aligned}
%     \kern -0.3cm\dot{H}(\mathbf{x}) =& \left(\kern -0.1cm\frac{\partial \calH(\mathbf{x})}{\partial \mathbf{x}}\kern -0.1cm\right)^T\kern -0.3cm\dot{\mathbf{x}} = \\& \left(\kern -0.1cm\frac{\partial \calH(\mathbf{x})}{\partial \mathbf{x}}\kern -0.1cm\right)^T\kern -0.3cm\left( \mathbf{J}(\mathbf{x}) \kern -0.1cm   - \kern -0.1cm  \mathbf{R}(\mathbf{x})\right)
% \frac{\partial {H}(\mathbf{x})}{\partial\mathbf{x}}. 
% \end{aligned}
% \end{equation}
% Therefore, if $( \mathbf{J}(\mathbf{x})   -   \mathbf{R}(\mathbf{x})) \preceq \mathbf{0}$ and $\frac{\partial {H}(\mathbf{x})}{\partial\mathbf{x}} \neq \mathbf{0}$ for all configurations except the equilibrium, where $\partial {H}(\mathbf{x}) / \partial\mathbf{x} = \mathbf{0}$, then the system is stable in the sense of Lyapunov. First, $  \mathbf{R}(\mathbf{x}) \succeq \mathbf{0}$ by definition of the port-Hamiltonian system. Second, $  \mathbf{J}(\mathbf{x})$ is skew-symmetric by definition of the port-Hamiltonian system, so
% \begin{equation}\label{eq:Jskew}
% \begin{aligned}
%     A =& \frac{\partial \calH(\mathbf{x})}{\partial \mathbf{x}}^T \mathbf{J}(\mathbf{x}) \frac{\partial \calH(\mathbf{x})}{\partial \mathbf{x}} \in \mathbb{R} \quad \text{(scalar)},
%     \\
%     A^T =&  \frac{\partial \calH(\mathbf{x})}{\partial \mathbf{x}}^T \mathbf{J}^T(\mathbf{x}) \frac{\partial \calH(\mathbf{x})}{\partial \mathbf{x}} = -A.
% \end{aligned}
% \end{equation}
% Therefore, $A = 0$ and $\dot{H}(\mathbf{x}) \leq 0$. If $\partial {H}(\mathbf{x}) / \partial\mathbf{x} = \mathbf{0}$, then the system is stable in the sense of Lyapunov, concluding the proof. 
% \end{proof}

% In turn, the IDA-PBC guarantees stability if the port-Hamiltonian constraints hold and we ensure that, at equilibrium, $\mathbf{J}(\mathbf{x}), \mathbf{R}(\mathbf{x})$ and ${H}(\mathbf{x})$ are zero. Nevertheless, it is important to remark that, to fulfill the conditions in Proposition~\ref{prop:stability} \textbf{and} achieve the task, the equilibrium of the observed and learned closed-loop dynamics must be the same\NA{This is vague. We did not define what ``an equilibrium'' means and how the equilibria of the learned and demonstrated closed-loop systems correspond. We should either remove this or make it more precise by introducing the Hamiltonian $H^*(\mathbf{x})$ resulting from the true policy and discussing the relationship between $\arg\min_{\mathbf{x}} H^*(\mathbf{x})$ and $\arg\min_{\mathbf{x}} \calH(\mathbf{x})$.}; otherwise, despite converging, there is no guarantee that the learned control policy drives the system towards the correct equilibrium. Besides, if the port-Hamiltonian terms are computed in a distributed fashion, then the learning problem is successfully moved from an unstructured learning problem within a large class of control policies to a structured learning problem within a tighter class of control policies that guarantee stability and a distributed architecture. In the next Subsection we propose a solution to learn $\mathbf{R}(\mathbf{x}), \mathbf{J}(\mathbf{x})$ and ${H}(\mathbf{x})$ such that they respect both the port-Hamiltonian, stability and distributed constraints. 

\begin{example}\label{example:portHamiltonian}
The closed-loop dynamics of the flocking is
\begin{equation}\label{eq:closed_loop_new}
        \dot{{\mathbf{s}}} = {\mathbf{v}}, \qquad 
        \dot{{\mathbf{v}}} = -\frac{\partial {U}({\mathbf{s}})}{\partial{\mathbf{s}}} - \mathbf{D}({\mathbf{s}}){\mathbf{v}}.
\end{equation}
Moreover, $\mathbf{F}_s(\mathbf{x}) = [\mathbf{0}, \mathbf{I}]^T$. The terms in Eq.~\eqref{eq:closed_loop_new} read
\begin{align}\label{eq:potentials1}
     \frac{\partial {U}({\mathbf{s}})}{\partial{\mathbf{s}}_i}  =&  c_1{\mathbf{s}}_i + \sum_{j \in \mathcal{N}_i}  \phi(||{\mathbf{s}}_{j}-{\mathbf{s}}_i||_{\sigma})\mathbf{n}_{ij},\!\\
     [\mathbf{D}({\mathbf{s}})]_{ij}  =&  \left(  c_2 [\mathbf{I}_n]_{ij}  +  \rho \left(||{\mathbf{s}}_{j}-{\mathbf{s}}_i||_{\sigma}/\tau\right) \right) \mathbf{I}_m,
\end{align}
so 
% \begin{equation}\label{eq:closed_loop_Ham}
%         \kern -0.4cm\begin{pmatrix}
%         \dot{{\mathbf{s}}} \\ \dot{{\mathbf{v}}}
%         \end{pmatrix}
%         = \prl{\bfJ - \bfR} \begin{pmatrix}
%         \frac{\partial {H}({\mathbf{s}}, {\mathbf{v}})}{\partial{\mathbf{s}}}\\ \frac{\partial {H}({\mathbf{s}}, {\mathbf{v}})}{\partial{\mathbf{v}}}
%         \end{pmatrix},
% \end{equation}
$\bfJ =          \begin{pmatrix}
        \mathbf{0} & \kern -0.2cm \mathbf{I}_n\\ -\mathbf{I}_n & \kern -0.2cm\mathbf{0}
        \end{pmatrix}$, $\bfR =          \begin{pmatrix}
        \mathbf{0} &  \mathbf{0}\\ \mathbf{0} &  \mathbf{D}({\mathbf{s}})
        \end{pmatrix}$, and ${H}({\mathbf{s}},{\mathbf{v}}) = {U}({\mathbf{s}}) + \frac{1}{2}{\mathbf{v}}^T{\mathbf{v}}$.
\end{example}


% \begin{equation}\label{eq:open_loop}
% \begin{aligned}
%         \dot{\mathbf{v}} &= - \mathcal{F}(\mathbf{x})\mathcal{F}_u^T(\mathbf{x})\frac{\partial \mathcal{H}_u(\mathbf{x})}{\partial \mathbf{x}}
% \\
% &= \left(\mathcal{J}_u(\mathbf{x}) - \mathcal{R}_u(\mathbf{x})\right)\frac{\partial \mathcal{H}_u(\mathbf{x})}{\partial\mathbf{x}}.
% \end{aligned}
% \end{equation}
% If $\mathcal{F}_u = \mathbf{I}$, $\mathcal{J}_u = \mathbf{0}$ and $\mathcal{F} = \mathcal{R}_u$, then Eq.~\eqref{eq:open_loop} holds.
% % \begin{equation}\label{eq:open_loop_intro_controller2}
% %         \mathbf{u} = -\mathcal{F}_s^{\dagger}\left(\left(\mathcal{J}_s(\mathbf{x}) - \mathcal{R}_s(\mathbf{x})\right)\frac{\partial \mathcal{H}_s(\mathbf{x})}{\partial\mathbf{x}}\left(\frac{\partial \mathcal{H}_u(\mathbf{x})}{\partial\mathbf{x}}\right)^{\ddagger} + \left(\mathcal{J}(\mathbf{x}) - \mathcal{R}(\mathbf{x})\right)\frac{\partial \mathcal{H}(\mathbf{x})}{\partial\mathbf{x}}\left(\frac{\partial \mathcal{H}_u(\mathbf{x})}{\partial\mathbf{x}}\right)^{\ddagger}\right)
% % \end{equation}
% The interconnection of two port-Hamiltonian systems is also a port-Hamiltonian system~\cite{shaft2004port}, with total energy $\mathcal{H}(\mathbf{x}) = \frac{1}{2}\mathbf{v}^T\mathbf{v} + \mathcal{H}_u(\mathbf{x})$. Therefore, 

% Note that $\partial \mathcal{H}(\mathbf{x}) / \partial\mathbf{v} = \mathbf{v}$, which implies that $\mathcal{H}_u(\mathbf{x}) = \mathcal{H}_u(\mathbf{p})$ and therefore $\partial \mathcal{H}(\mathbf{x}) / \partial\mathbf{p} = \partial \mathcal{H}_u(\mathbf{p}) / \partial\mathbf{p}$. 
 

% Last but not least, if constraints $\mathcal{R}(\mathbf{x}) \succeq \mathbf{0}$ and $\mathcal{H}(\mathbf{x}) \geq 0$ are enforced, then the system is stable, and so the control policy does not destabilize the system by construction.





% \ES{At this point of the research, we might need to discuss what do we really want to propose as solution. Some tips: (i) If the solution (Steps 1 and 2) receives, as input, the whole state, then even if we use the Boolean Laplacian to constraint the training, then the policy is not distributed. On the other hand, Step 3 yields to a distributed policy, so in a realistic deployment, only Step 3 is affordable. Therefore, Steps 1 and 2 remain an identification solution, while Step 3 obtains a really implementable policy; (ii) Step 1 is a bit unrealistic because we could obtain a $\tau$ that does not correspond to the actual messages a robot is receiving during deployment; (iii) If the solution works online, then the loss function should reflect not only the error between predicted and actual, but also the control objective itself; (iv) for sure that the solution can be embedded in a RL framework (see PettingZoo slides), but this may be a future step. Afterwards, we could use Isaac Gym} 

\subsection{Learning Distributed Multi-Robot Interactions}\label{subsec:LEMURS}

In Sec.~\ref{subsec:portHamiltonian} we have reduced  problem~\eqref{eq:prob_def} to learning $\mathbf{J}(\mathbf{x})$, $\mathbf{R}(\mathbf{x})$ and ${H}(\mathbf{x})$. For brevity, let $\mathbf{X}_i = [\mathbf{x}_{i}, \mathbf{x}_{j_1}, \mathbf{x}_{j_2}, \hdots, \mathbf{x}_{j_{|\mathcal{N}_i|}}].$  According to the requirements in \eqref{eq:JRH_conditions}, we design the port-Hamiltonian terms such that they only depend on neighboring information:
% \begin{equation} \label{eq:individual_terms}
%     \begin{aligned}
%         \calH(\mathbf{x}) =& \sum_{i=0}^n H^{(i)}(\mathbf{x}^a_i) \\
%         [\mathbf{J}(\mathbf{x})]_{i} =& \mathbf{J}^{(i)}(\mathbf{x}^a_i), \quad \forall i\\
%         [\mathbf{R}(\mathbf{x})]_{i} =& \mathbf{R}^{(i)}(\mathbf{x}^a_i), \quad \forall i
%     \end{aligned}
% \end{equation}
\begin{gather} \label{eq:individual_terms}
        \kern -0.5cm [\mathbf{J}_{\mathbf{p}\mathbf{q}}]_{ii} = \mathbf{J}^{(i,i)}_{\mathbf{p}\mathbf{q}}(\mathbf{X}_i, \bm{\theta_J}), \hbox{ } [\mathbf{J}_{\mathbf{q}\mathbf{p}}]_{ii}  = \mathbf{J}^{(i,i)}_{\mathbf{q}\mathbf{p}}(\mathbf{X}_i, \bm{\theta_J}),
        \\ 
        \kern -0.4cm [\mathbf{R}_{\mathbf{p}\mathbf{p}}]_{ij} = \mathbf{R}^{(i,j)}_{\mathbf{\mathbf{p}\mathbf{p}}}(\mathbf{X}_i, \bm{\theta_R}),\hbox{ }
        [\mathbf{M}_{\mathbf{k}\mathbf{h}}]_{ij}= \mathbf{M}^{(i,j)}_{\mathbf{\mathbf{k}\mathbf{h}}}(\mathbf{X}_i,\bm{\theta}_H).
\end{gather}
The control policy is now parameterized by $\bm{\theta} := \{\bm{\theta_J}, \bm{\theta_R}, \bm{\theta}_H \}$.
% \begin{equation}\label{eq:open_loop_intro_controller_ind}
% \begin{aligned}
% \kern -0.2cm \mathbf{u}_i &= (\mathbf{F}_s^{(i)}(\mathbf{x}_i))^{\dagger}
% \left((\mathbf{J}^{(i)}(\mathbf{x}_i^a) - \mathbf{R}^{(i)}(\mathbf{x}_i^a) \frac{\partial H^{(i)}(\mathbf{x}_i^a)}{\partial\mathbf{x}_i^a}-\right.
% \\
% & \qquad \qquad \qquad \left.(\mathbf{J}_s^{(i)}(\mathbf{x}_i) - \mathbf{R}_s^{(i)}(\mathbf{x}_i)) \frac{\partial {H}_s^{(i)}(\mathbf{x}_i)}{\partial\mathbf{x}_i}\right).
% \end{aligned}
% \end{equation}
% From Eqs.~\eqref{eq:open_loop_intro_individual} and \eqref{eq:open_loop_intro_controller_ind}, the control policy yields to the robot $i$ closed-loop dynamics 
% \begin{equation}\label{eq:individual_dynamics}
%     \dot{\mathbf{x}}_i = \sum_{j \in \mathcal{N}_i \cup \{i\}}([\mathbf{J}(\mathbf{x}_i^a)]_{ij}-[\mathbf{R}(\mathbf{x}_i^a)]_{ij})\frac{\partial \calH(\mathbf{x})}{\partial \mathbf{x}_j}.
% \end{equation}
% The unknown terms $[\mathbf{J}(\mathbf{x}_i^a)]_{ij}, [\mathbf{R}(\mathbf{x}_i^a)]_{ij}$ and $\frac{\partial \calH(\mathbf{x})}{\partial \mathbf{x}_j}$ must be computed from local information only, and the stability and distributed conditions must hold. 
% Besides, it is desirable to find a way of learning  $[\mathbf{J}(\mathbf{x})]_{ij}, [\mathbf{R}(\mathbf{x})]_{ij}$ and $\frac{\partial H_i(\mathbf{x})}{\partial \mathbf{x}_j}$ such that, if they are implemented in a team with a time-varying number of robots\NA{Save this for the experiments section. So far our problem formulation has not considered $n$} or the graph topology changes with time, then the task is still accomplished. 
These terms are learned by means of a novel architecture based on the principles of self-attention~\cite{vaswani2017attention}. 

% :
% \begin{equation}\label{eq:individual_dynamics_parameters}
%     \kern -0.2cm\dot{\mathbf{x}}_i \kern -0.1cm = \kern -0.4cm \sum_{j \in \mathcal{N}_i \cup \{i\}}\kern -0.2cm([\mathbf{J}(\mathbf{x}_i^a, \bm{\theta_J})]_{ij}\kern -0.1cm-\kern -0.1cm[\mathbf{R}(\mathbf{x}_i^a, \bm{\theta_R})]_{ij})\frac{\partial \calH(\mathbf{x},\bm{\theta}_H)}{\partial \mathbf{x}_j}.
% \end{equation}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Images/FigureArchitecture.png}
    \caption{Proposed architecture for LEMURS.}
    \label{fig:architecture}
\end{figure}


To learn $\mathbf{R}^{(i,j)}_{\mathbf{\mathbf{p}\mathbf{p}}}(\mathbf{X}_i, \bm{\theta_R})$, robot $i$ receives, at instant $t$, the state from its neighbors $j \in \mathcal{N}_i$. Together with its own state, the information is processed via 
\begin{align}\label{eq:selfattention}
        &\kern -5pt\mathbf{X}_i^1 = [\mathbf{x}_{i},     \mathbf{x}_{j_1}, \mathbf{x}_{j_2}, \hdots, \mathbf{x}_{j_{|\mathcal{N}_i|}}]
        \\
        &\kern -0.2cm\kern -5pt\text{ for }w=1,\hdots, W:
        \\
        &\kern -0.2cm \mathbf{Q}_i^w =  \mathbf{A}^w_{Q,\mathbf{R}}{\mathbf{X}}_i^w, \hbox{ } \mathbf{K}_i^w = \mathbf{A}^w_{K,\mathbf{R} }\mathbf{X}_i^w, \hbox{ } \mathbf{V}_i^w = \mathbf{A}^w_{V,\mathbf{R}}\mathbf{X}_i^w, 
    \\
    &\kern -0.2cm\mathbf{Y}_i^w = \gamma\left(\mathsf{softmax}\left(\frac{\beta(\mathbf{Q}^w_i)\beta((\mathbf{K}_i^w)^T)}{\sqrt{|\mathcal{N}_i|}}\right) \beta(\mathbf{V}_i^w)\right),
    \\
    &\kern -0.2cm\mathbf{X}_i^w = \alpha^2(\mathbf{A}^w_{Z, \mathbf{R}}{\mathbf{Y}}_i^w).\label{eq:selfattention2}   
\end{align}
$W$ is the number of self-attention layers; $\mathbf{A}^w_{Q, \mathbf{R}}, \mathbf{A}^w_{K, \mathbf{R}}, \mathbf{A}^w_{V, \mathbf{R}} \in \mathbb{R}^{r_w \times h_w}$ and $\mathbf{A}^w_{Z, \mathbf{R}} \in \mathbb{R}^{d_w \times r_w}$ $\forall w$ are matrices to be learned and shared across robots; meanwhile, $\mathbf{Z}_i = \mathbf{X}_i^W\in \mathbb{R}^{d_w \times |\mathcal{N}_i \cup \{i\}|}$ is the output, with $h_w, r_w, d_w>0$. The size of $\mathbf{A}^w_{Q, \mathbf{R}}, \mathbf{A}^w_{K, \mathbf{R}}, \mathbf{A}^w_{V, \mathbf{R}}$ does not depend on the number of robots, so robot $i$ can deal with time-varying neighbors. Nonlinear activation functions $\beta(\cdot)$, $\gamma(\cdot)$ and $\alpha(\cdot)$ account for potential nonlinearities. 
% \TD{Maybe I missed something here but how does $n$ appears here while $\mathbf{X}_i \in \mathbb{R}^{n_x \times |\mathcal{N}_i + 1|}$?} \ES{Typo, corrected}.
Then,  $\mathbf{R}^{(i,j)}_{\mathbf{\mathbf{p}\mathbf{p}}}(\mathbf{X}_i, \bm{\theta_R})$ is
\begin{gather}\label{eq:Restimate}
    \begin{aligned}
    \relax [{\mathbf{Z}}^a_i]_{j} =& \mathsf{vec}^{-1}([{\mathbf{Z}}_i]_{j}),
    \\
    \mathbf{R}^{(i,j)}_{\mathbf{\mathbf{p}\mathbf{p}}}(\mathbf{X}_i, \bm{\theta_R}) =& -([{\mathbf{Z}}^a_i]_{j}+[{\mathbf{Z}}^a_j]_{i}), \quad  \forall j \in \mathcal{N}_i,
    \\
    \mathbf{R}^{(i,i)}_{\mathbf{\mathbf{p}\mathbf{p}}}(\mathbf{X}_i, \bm{\theta_R}) =& [{\mathbf{Z}}^a_i]_{i} +  \sum_{j \in \mathcal{N}_i}  ([{\mathbf{Z}}^a_i]_{j}+[{\mathbf{Z}}^a_j]_{i}),
    \end{aligned}
\end{gather}
where $\mathsf{vec}^{-1}(\cdot)$ is the operator that reshapes the $d_W \times 1$ vector to a $n_x \times n_x$ matrix. The steps in~\eqref{eq:Restimate} ensure that 
%$\hat{\mathbf{R}}(\mathbf{x}) \in \mathsf {wspace}(\mathbf{L})$; this implies that 
${\mathbf{R}}(\mathbf{x}) \succeq \mathbf{0}$ by construction. 
% a row vector ${\mathbf{a}}_i$ and a scalar ${{a}}_i$ are computed
% \begin{equation}\label{eq:adjacency}
% \begin{aligned}
%     \relax[{\mathbf{a}}_i]_{j} =& \gamma((\mathbf{w}^R_{j})^T \mathbf{y}^R_i)^2  \hbox{ } \forall j \in \mathcal{N}_i, \hbox{ and $0$ otherwise},
%     \\
%     {{a}}_i =& \gamma((\mathbf{w}^R_{i})^T\mathbf{y}_i)^2.
% \end{aligned}
% \end{equation}
% Here, $\gamma(\cdot)$ is a nonlinear activation function. Finally,
%  . 

Regarding $\mathbf{J}^{(i,i)}_{\mathbf{p}\mathbf{q}}(\mathbf{X}_i, \bm{\theta_J})$ and $\mathbf{J}^{(i,i)}_{\mathbf{q}\mathbf{p}}(\mathbf{X}_i, \bm{\theta_J})$, similar steps can be followed. Steps~\eqref{eq:selfattention}-\eqref{eq:selfattention2} are the same, with parameters $\mathbf{A}^w_{Q, \mathbf{J}}, \mathbf{A}^w_{K, \mathbf{J}}, \mathbf{A}^w_{V, \mathbf{J}}$ and $\mathbf{A}^w_{Z, \mathbf{J}}$; then, the skew-symmetry is imposed, $$\mathbf{J}^{(i,i)}_{\mathbf{p}\mathbf{q}}(\mathbf{X}_i, \bm{\theta_J}) = - \mathbf{J}^{(i,i)}_{\mathbf{q}\mathbf{p}}(\mathbf{X}_i, \bm{\theta_J}) = ({\mathbf{Z}}_i^a)^T - {\mathbf{Z}}_i^a.$$ 

Regarding $\mathbf{M}^{(i,j)}_{\mathbf{\mathbf{k}\mathbf{h}}}(\mathbf{X}_i,\bm{\theta}_H)$ and $P^{(i)}(\mathbf{X}_i,\bm{\theta}_H)$,  similar steps can be followed. Steps~\eqref{eq:selfattention}-\eqref{eq:selfattention2} are the same, with parameters  $\mathbf{A}^w_{Q, \mathbf{M}}, \mathbf{A}^w_{K, \mathbf{M}}, \mathbf{A}^w_{V, \mathbf{M}}$,  $\mathbf{A}^w_{Z, \mathbf{M}}$ and $\mathbf{A}^w_{Q, U}, \mathbf{A}^w_{K, U}, \mathbf{A}^w_{V, U}$, $\mathbf{A}^w_{Z, U}$; then, we apply~\eqref{eq:Restimate} to obtain $\mathbf{M}^{(i,j)}_{\mathbf{\mathbf{k}\mathbf{h}}}(\mathbf{X}_i,\bm{\theta}_H)$ instead of $\mathbf{R}^{(i,j)}_{\mathbf{\mathbf{p}\mathbf{p}}}(\mathbf{X}_i, \bm{\theta_R})$. Finally, the Hamiltonian is computed such that
\begin{equation}\label{eq:Hestimate}
\begin{aligned}
    &{H}_i(\mathbf{X}_i) = \sum_{\mathbf{k}, \mathbf{h} \in \{\mathbf{p}, \mathbf{q}\}} \sum_{j \in \mathcal{N}_i \cup \{ i \}} \mathbf{k}_j^T \mathbf{M}^{(i,j)}_{\mathbf{\mathbf{k}\mathbf{h}}}(\mathbf{X}_i,\bm{\theta}_H) \mathbf{h}_j + {U}_i(\mathbf{X}_i),
    \\
    &{U}_i(\mathbf{X}_i) = \mathbf{1}^T\mathbf{Z}^U_i\mathbf{1}.
\end{aligned}
\end{equation}
Here, $(\mathbf{x}^a_i)^T \mathbf{M}_i(\mathbf{X}_i)\mathbf{x}^a_i$ and ${U}_i(\mathbf{X}_i)$ play the role of kinematic and potential energy respectively. Finally, the automatic differentiation tool in PyTorch~\cite{paszke2019pytorch} is used to obtain $\partial \hat{H}(\mathbf{x})/\partial \mathbf{x}_j$. 

We define $$\hat{\mathcal{F}}_i = \{ [\hat{H}(\mathbf{x})]_j,[\hat{\mathbf{R}}(\mathbf{x}_i^a)]_{ij}, [\hat{\mathbf{J}}(\mathbf{x}_i^a)]_{ij} \}_{j\in \mathcal{N}_i \cup \{i\}}$$ and  
$$
\hat{\mathcal{F}}_i =  \mathsf{SA}(\mathbf{X}_i,\bm{\theta}),
$$where \textsf{SA} denotes the operations from~\eqref{eq:selfattention} to~\eqref{eq:Hestimate} and $$\bm{\theta} = \{ \{\mathbf{A}^w_{Q, k}, \mathbf{A}^w_{K, k}, \mathbf{A}^w_{V, k}, \mathbf{A}^w_{Z, k}\}_{w=1}^{w=W}\}_{k=\mathbf{R,J},H}.$$
% Importantly,~\eqref{eq:Hestimate} implies that, if $\mathbf{X}_i = \mathbf{0}$ \TD{In Sec 3A, we talked about stability around $\bfx^*$ with  $\partial {H}(\mathbf{x})/ \partial \mathbf{x} = 0$ and ${H}(\mathbf{x}) = 0$. Here, it seems like $\bfx^* = 0$. Should we clarify here that the state can be offset by $\bfx^*$ to move the equilibrium to $0$? This is more consistent with the offset network input in the Appendix.}, then both $\partial {H}(\mathbf{x})/ \partial \mathbf{x}$ and ${H}(\mathbf{x})$ are zero, which fulfills the stability requirements.
% \TD{Why }\ES{Typo from previous versions, corrected}.

The training process is conducted by solving the following optimization problem, coined as LEMURS (\textbf{LE}arning distributed \textbf{MU}lti-\textbf{R}obot interaction\textbf{S}) 
\begin{subequations}\label{eq:step2}
\begin{alignat}{2}
\kern -1cm \underset{\bm{\theta}}{\min} & \hbox{ }       \mathcal{L}(\mathbf{x}_{0:K},\hat{\mathbf{x}}_{0:K}) \label{eq:step2cost}
\\
s.t. &  \hbox{ }\hat{\mathbf{x}}(0) = \mathbf{x}(0) = \mathbf{x}_0\label{eq:step2constraint1}
\\
& \hbox{ }\hat{\mathcal{F}}_i = \mathsf{SA}(\mathbf{X}_i,\bm{\theta}) \hbox{ } \forall i,t\label{eq:step2constraint2}
\\
& \hbox{ }\hat{\mathbf{x}}_{1:K} = \mathsf{ODEsolver}(\hbox{Eq.}~\eqref{eq:closed_loop_intro}, \mathbf{x}_0, \mathbf{L}_{0:K}, \bm{\theta}, \hat{\mathcal{F}}) \label{eq:step2constraint3}
\end{alignat}
\end{subequations}


According to constraint~\eqref{eq:step2constraint2}, the estimated states are calculated by an ordinary differential equation solver and the gradient of the loss function is back-propagated using adjoint methods~\cite{chen2018neural}. The parameters $\bftheta$ are updated using gradient descent.
% Besides, note that the parameters $\bm{\theta}$ are shared across robots and the control policy does not depend on the number of robots in the team, so it is scalable to any robot team size. This is a significant difference with other approaches like multi-layer perceptrons and graph neural networks, where the size of the layers/filters depends on the number of robots, it is much more trickier to scale the policies.




\begin{example}\label{example:flockingsolution}
In the case of flocking, LEMURS can be directly applied to learn $\mathbf{D}(\mathbf{p})$ and ${U}(\mathbf{p})$. Another option is to learn $\mathbf{J}(\mathbf{x}), \mathbf{R}(\mathbf{x})$ and ${H}(\mathbf{x})$ and use the IDA-PBC, obtaining extra degrees of freedom for the control policy. In this sense, $\mathbf{J}(\mathbf{x}), \mathbf{R}(\mathbf{x})$ and ${H}(\mathbf{x})$ can be either dense or sparse/block-sparse matrices. The former implies more degrees of freedom while the latter can be used to, e.g., reduce the number of potential underdamped modes of the learned policy.
\end{example}





==> 06_Simulations.tex <==

In this section we evaluate LEMURS in three multi-robot tasks in simulation, illustrated in Fig.~\ref{fig:examples}:
\begin{enumerate}
    \item \emph{Fixed swapping} \cite{furieri2021distributed}: Robots are initialized in two columns and navigate to the diagonally opposite position in the other column while avoiding collisions (Fig.~\ref{fig:fixedswapping_gtc}). The communication graph is a fixed ring such that robot $i$ communicates with robots $(i\pm1)\mod n$. We use the same parameters as~\cite{furieri2021distributed}. We generate demonstrations from the following expert controller:
    \begin{equation} \label{eq:swapping-expert}
            \mathbf{u}_i = -c_1\mathbf{p}_i-c_2\mathbf{v}_i - \sum_{j\in\mathcal{N}_i^1}\frac{\mathbf{p}_{i}-\mathbf{p}_{j}}{\sqrt{1+\sigma||\mathbf{p}_{i}-\mathbf{p}_{j}||^2_2}},
    \end{equation} with $c_1=0.8$, $c_2=1.0$, $\sigma = 0.1$.
    %The parameters are in Furieri et al.~\cite{furieri2021distributed}.
    
    \item \textit{Time-varying swapping}: We consider the \textit{fixed swapping} task but with a time-varying communication graph (Fig.~\ref{fig:tvswapping_gtc}), where $\mathbf{A}(t)$ is such that $[\mathbf{A}(t)]_{ij} = \mathsf{sigmoid}(\lambda(||\mathbf{p}_i(t)-\mathbf{p}_j(t)|| - l/2))$ if $||\mathbf{p}_i(t)-\mathbf{p}_j(t)||<l$ and $0$ otherwise, with $l = 2.4$m and $\lambda = 2.0$. We use the controller in \eqref{eq:swapping-expert} with time-varying neighbors to generate demonstrations.
    
    \item \textit{Flocking}: We consider the flocking task described in Examples~\ref{example:flocking_controller}-\ref{example:flockingsolution} with parameters from \cite{olfati2006flocking} (Fig.~\ref{fig:flocking_gtc}). We use the controller \eqref{eq:real_flocking_controller} in to generate demonstrations. 
\end{enumerate}

% We generate datasets from the following expert controllers:
% \begin{enumerate}
%     \item \textit{Fixed swapping} and \textit{time-varying swapping}: 
%     \begin{equation*}
%             \mathbf{u}_i = -c_1\mathbf{p}_i-c_2\mathbf{v}_i - \sum_{j\in\mathcal{N}_i^1}\frac{\mathbf{p}_{i}-\mathbf{p}_{j}}{\sqrt{1+\sigma||\mathbf{p}_{i}-\mathbf{p}_{j}||^2_2}},
%     \end{equation*} with $c_1=0.8$, $c_2=1.0$, $\sigma = 0.1$.
%     \item \textit{Flocking}: Eq. \eqref{eq:real_flocking_controller} in Example~\ref{example:flocking_controller}.
% \end{enumerate}


The training and evaluation datasets for each task are formed by $L=400$ trajectories of $K=250$ samples with sampling interval $T=0.04$s. The number of demonstrating robots is $n=4$, and the trajectories are split in sub-trajectories of $5$ samples for training. We train the self-attention Hamiltonian neural ODE networks for $10000$ epochs with the Euler numerical method \cite{butcher2016numerical}, learning rate $\eta = 0.001$, and new batches of $200$ samples every $100$ epochs. We consider $k = 1$ as the number of hops.

The learned control policies are stable and scalable for all the tasks, converging to the desired goal with a larger number of robots as seen in Figs.~\ref{fig:examples}. We plot trajectories from the expert control policy (left) for $4$ training robots and learned control policies for $n=12$ robots (right), three times larger than the team size in training. Similar results with up to $64$ robots can be found on our website\footnote{\scriptsize \url{https://eduardosebastianrodriguez.github.io/LEMURS/}}.  LEMURS successfully captures complex behaviors that are not encoded a priori, such as the collision avoidance or the flock formation in \textit{flocking}. Since we train LEMURS for \emph{flocking} with only $4$ robots in Fig. \ref{fig:flocking_gtc}, LEMURS infers that it is desired to have $4$ groups of robots with equal inter-robot distances between the groups (Fig. \ref{fig:flocking_lcp}), instead of having equal robot distances among the $12$ robots. To improve generalization, we suggest increasing the number of robots during training since LEMURS training is scalable, but we leave this investigation for future work. Furthermore, the learned control policies in the \emph{swapping} tasks are less suboptimal than the expert controller as seen in Fig. \ref{fig:fixedswapping_lcp}~and~\ref{fig:tvswapping_lcp}. As the training dataset is formed by short sub-trajectories of $5$ samples, which resemble a straight line in general, LEMURS infers that the motion to the goals should be a straight line as well. 

\begin{figure}[!ht]
    \centering\hspace{-0.6cm}
    \begin{tabular}{cc}
    \subcaptionbox{Fixed swapping, ECP\label{fig:fixedswapping_gtc}}
      {\includegraphics[width=0.48\columnwidth]{Images/FixedSwapping.png}}
      &  
    \subcaptionbox{Fixed swapping, LCP\label{fig:fixedswapping_lcp}}
      {\includegraphics[width=0.48\columnwidth]{Images/FixedSwappingResult.png}}
      \\
    \subcaptionbox{TV swapping, ECP\label{fig:tvswapping_gtc}}
      {\includegraphics[width=0.48\columnwidth]{Images/TvSwapping.png}}
      &
    \subcaptionbox{TV swapping, LCP\label{fig:tvswapping_lcp}}
      {\includegraphics[width=0.48\columnwidth]{Images/TvSwappingResult.png}}
      \\
    \subcaptionbox{Flocking, ECP\label{fig:flocking_gtc}}
      {\includegraphics[width=0.48\columnwidth]{Images/Flocking.png}}
      &
    \subcaptionbox{Flocking, LCP\label{fig:flocking_lcp}}
      {\includegraphics[width=0.48\columnwidth]{Images/FlockingResult.png}}
    \end{tabular}
	\caption{\small Demonstration of expert and learned control policies: (left) expert control policies (ECP) for training with $4$ robots, (right) learned control policies (LCP) with $12$ robots for $3$ tasks.
% 	: \emph{fixed swapping} (top), \emph{time-varying (TV) swapping} (middle), and \emph{flocking} (bottom)
	}
	\label{fig:examples}
\end{figure}

%To show the effectiveness of LEMURS, w
We compare LEMURS with three other learning methods: 1) Multi-Layer Perceptron (MLP), inspired by~\cite{furieri2021distributed}; 2) Graph Neural Network (GNN) from~\cite{khan2020graph,yang2021communication}; and 3) Self-Attention based Graph Neural Network (GNNSA)~\cite{li2021message}. These learning models substitute the self-attention layers in our Hamiltonian-based neural ODE networks. The size of the layers/filters in the MLP, GNN and GNNSA depends on the number of robots, so scalability is not directly achievable unlike in our approach. Our LEMURS has $2208$ parameters while MLP, GNN and GNNSA have $1$ layer/filter with $4448, 4448$ and $4672$ parameters, respectively. The implementation details are in the Appendix~\ref{sec:parameters}. 

\begin{figure}[!ht]
    \centering\hspace{-0.6cm}
    \begin{tabular}{cc}
    \subcaptionbox{Fixed swapping, training}
      {\includegraphics[width=0.48\columnwidth]{Images/FixedSwappingTraining.png}}
      &  
    \subcaptionbox{Fixed swapping, scalability}
      {\includegraphics[width=0.48\columnwidth]{Images/FixedSwappingScalability.png}}
      \\
    \subcaptionbox{TV swapping, training}
      {\includegraphics[width=0.48\columnwidth]{Images/TvSwappingTraining.png}}
      &
    \subcaptionbox{TV swapping, scalability}
      {\includegraphics[width=0.48\columnwidth]{Images/TvSwappingScalability.png}}
      \\
    \subcaptionbox{Flocking, training\label{fig:training_flocking}}
      {\includegraphics[width=0.48\columnwidth]{Images/FlockingTraining.png}}
      &
    \subcaptionbox{Flocking, scalability}
      {\includegraphics[width=0.48\columnwidth]{Images/FlockingScalability.png}}
    \end{tabular}
	\caption{\small LEMURS training scalability and comparison with a multi-layer perceptron (MLP)~\cite{furieri2021distributed}, a graph neural network (GNN)~\cite{khan2020graph,yang2021communication} and a self-attention-based graph neural network (GNNSA)~\cite{li2021message} in learning robot interactions: (left) training loss over $10000$ epochs, (right) LEMURS training scalability with $4, 8, 16$ robots for $3$ tasks.
% 	: \emph{fixed swapping} (top), \emph{time-varying (TV) swapping} (middle), and \emph{flocking} (bottom).
	}
	\label{fig:training_and_scalability}
\end{figure}

Fig.~\ref{fig:training_and_scalability} (left) plots the mean and standard deviation of the training loss of the $4$ models and the $3$ tasks, from $3$ runs using $3$ randomized seeds. Our self-attention architecture surpasses the other three methods in capturing interactions for all tasks with half of the number of parameters, illustrating the benefits of combining self-attention networks and Hamiltonian architecture in LEMURS. For tasks with time-varying topologies, i.e. \emph{time-varying swapping} and \emph{flocking}, LEMURS achieves training loss two orders of magnitudes better than that of MLP, GNN and GNNSA. Meanwhile, the MLP training did not converge with data from \emph{flocking} task. For \textit{fixed swapping} task with fixed topology, LEMURS's training loss is slightly better than that of GNNSA, and two orders of magnitudes better than that of MLP and GNN. 

% is the simplest multi-robot task, so LEMURS is only slightly better than the others. In examples with time-varying topologies, LEMURS is two orders of magnitude better than the second best method. In fact, the trace of the MLP does not appear in Fig.~\ref{fig:training_flocking} because the MLP is not able to learn the \textit{flocking} interactions. The results suggest that the other three models need larger and deeper architectures to obtain comparable results. 

%: for each one, randomly-initialized full-trajectory simulations of $4, 8, 16, 32, 64$ robots are conducted, $5$ runs per robot team size

We validate the scalability of the learned control policies for the three tasks. The policies are simulated over a time horizon $KT = 10$s. We train LEMURS with datasets of $4$, $8$ and $16$ robots, for $5$ runs using randomized seeds, and test the learned control policies with $4, 8, 16, 32, 64$ robots. The mean and standard deviation of the test loss (Eq.~\eqref{eq:loss_function}) is normalized by the number of robots, and plotted in Fig.~\ref{fig:training_and_scalability} (right). In general, our approach obtains similar test loss with respect to the number of training robots. In the case of \textit{fixed swapping}, increasing the number of robots in training improves the controller performance since the larger number of robots is, the more data there is for LEMURS to learn about a fixed communication topology.
For \textit{time-varying swapping} task, a small number of robots in training performs slightly better, potentially because the time-varying topology is more complex with more robots, i.e. it is harder to capture the robot interactions. Meanwhile, for \textit{flocking} task, increasing the number of training robots slightly improves the performance, even though the topology is also time-varying. This is because the robots form a flocking formation in the training trajectories, leading to a fixed topology in a large portion of the dataset, similar to \emph{fixed swapping}.



==> 08_Conclusions.tex <==
This work presented LEMURS, an algorithm that learns complex robot interactions from trajectory demonstrations using self-attention and Hamiltonian-based neural ODE networks. LEMURS advances the state of the art by learning control policies that time-varying communication and generalize to increasing numbers of robots. Our evaluation shows that LEMURS learns behaviors such as collision avoidance and flocking formation from state-only trajectories of few robots, and successfully replicates the tasks in a larger robot team. Future work will explore LEMURS in real-world tasks, where data is extracted from sensor observations and the learned control policies are deployed on real robots.


%the distributed control policy that replicates general multi-robot tasks. LEMURS learns the complex nonlinear interactions among robots from the demonstrations using self-attention techniques and Hamiltonian-based neural ODE networks, providing control policies that are distributed and scalable by construction. LEMURS  handles time-varying networks and time-varying numbers of robots, while avoiding potential unstable trajectories due to the port-Hamiltonian closed-loop guarantees. We verify the effectiveness of LEMURS on different tasks, showing that LEMURS can learn complex behaviors such as collision avoidance or flocking formations from state-only trajectories of few robots, and successfully achieve the tasks with larger robot team. Besides, LEMURS is shown to learn the task faster compared to other related approaches. Future work will explore LEMURS in real-world tasks, where data is extracted from, e.g., video sequences, and transferring the learned control policies to real robots.



==> 09_Flocking.tex <==
According to~\cite{olfati2006flocking}, in the flocking controller of Eq.~\eqref{eq:real_flocking_controller}:
\begin{align}\label{eq:potentials4}
    \phi(z) =& \rho(z/\tau)\psi(z-||d||_{\sigma})
\end{align}
is a potential function composed by
\begin{align}\label{eq:potentials5}
    \psi(z) :=\frac{(a+b)(z+c) + 1}{2(a+b)\sqrt{1+(z+c)^2}}
\end{align}
(with $0<a\leq b$, $c=\frac{\displaystyle|a-b|}{\displaystyle\sqrt{4ab}}$, $d>0$) and 
\begin{align}\label{eq:potentials6}
    \rho(z):=& \left \{ \begin{matrix}
    1, &  z\in(0,h)
    \\
    \frac{1}{2} \left[1+\cos\left(\pi \frac{\displaystyle z-h}{\displaystyle 1-h}\right) \right], &  z\in[h,1)
    \\
    0, &  \hbox{ otherwise,} 
    \end{matrix}\right.
\end{align}
with $h\in(0,1)$ and $\tau>0$. Besides, 
\begin{equation}\label{eq:potentials2}
    ||\mathbf{z}||_{\sigma} = \frac{1}{\sigma}(\sqrt{1+\sigma||\mathbf{z}||^2}-1)
\end{equation}
(with $\sigma>0$) is a smooth map of the 2-norm and
\begin{equation}\label{eq:potentials3}
    \mathbf{n}_{ij} = \frac{\mathbf{p}_{i}-\mathbf{p}_{j}}{\sqrt{1+\sigma||\mathbf{p}_{i}-\mathbf{p}_{j}||^2_2}}
\end{equation}
is the normalized vector between robots $i$ and $j$. In Eq.~\eqref{eq:potentials4}, $d$ is the desired inter-robot distance and $\tau$ is the communication radius.

==> 10_Networks.tex <==
The $\mathsf{SA}$ architecture is parameterized as follows:
\begin{itemize}
    % \item $[\mathbf{R}_{\bftheta}]_{ij}$: $W = 3$, $h_w=[4, 8, 8]$, $r_w = [8, 8, 8]$, $d_w = [8, 8, 16]$; $\beta(\cdot) = \mathsf{sigmoid}(\cdot)$, $\gamma(\cdot)=\alpha(\cdot)=\mathsf{swish}(\cdot)$~\cite{ramachandran2017searching}. 
    \item $[\mathbf{R}_{\bftheta}]_{ij}$: $W = 3$, $h_w=[4, 8, 8]$, $r_w = [8, 8, 8]$, $d_w = [8, 8, 16]$; functions $\beta = \mathsf{sigmoid}$, $\gamma=\alpha=\mathsf{swish}$~\cite{ramachandran2017searching}. 
    % The total number of parameters is $3\times(4 \times 8) + 2 \times 3 \times (8 \times 8) + 2 \times (8 \times 8) + (8 \times 16) = 736$.
    \item $[\mathbf{J}_{\bftheta}]_{ij}$: $W = 3$, $h_w=[4, 8, 8]$, $r_w = [8, 8, 8]$, $d_w = [8, 8, 1]$; functions $\beta = \mathsf{sigmoid}$, $\gamma=\alpha=\mathsf{swish}$~\cite{ramachandran2017searching}; and $[\mathbf{J}_{\bftheta}]_{ij} = \mathbf{0}$ $\forall i \neq j$.
    % The total number of parameters is $3\times(4 \times 8) + 2 \times 3 \times (8 \times 8) + 2 \times (8 \times 8) + (8 \times 16) = 736$.
    \item $H^{i}_{\bftheta}$: $W = 3$ layers, $h_w=[6, 8, 8]$, $r_w = [8, 8, 8]$, $d_w = [8, 8, 25]$; functions $\beta = \mathsf{sigmoid}$, $\gamma=\alpha=\mathsf{swish}$~\cite{ramachandran2017searching}. 
    % The total number of parameters is $3\times(6 \times 8) + 2 \times 3 \times (8 \times 8) + 2 \times (8 \times 8) + (8 \times 25) = 856$. 
\end{itemize}
The network input $\mathbf{X}_i^0$ is an offset version of \eqref{eq:concatenated_neighbors} as follows:
\begin{itemize}
    \item $[\mathbf{R}_{\bftheta}]_{ij}$ and $[\mathbf{J}_{\bftheta}]_{ij}$: $\mathbf{X}_i^0 = \brl{\Delta \bfx_{ii}, \{\Delta \bfx_{ij}\}_{j\in\calN_i^k\backslash\{i\}}}$.
    % \item : $[\mathbf{X}_i^0]_j = (\bfx_i - \bfx_j)$, $[\mathbf{X}_i^0]_i = (\bfx_i - \bar{\bfx}_i(KT))$.
    \item $H^{i}_{\bftheta}$: 
    $$\scaleMathLine{\mathbf{X}_i^0 = \brl{\{\Delta \bfx_{ii}, 0, 0\}, \{\Delta \bfx_{ij}, \Vert \Delta \bfx_{ij}\Vert^{\frac{1}{4}}_2, \Vert\Delta \bfx_{ij}\Vert_2\}_{j\in\calN_i^k\backslash\{i\}}},}$$
    % $[(\bfx_i - \bfx_j)^{\top}, 1/||\mathbf{x}_i-\mathbf{x}_j||_2^{-1/4}, ||\mathbf{x}_i-\mathbf{x}_j||_2]^{\top}$ and $[\mathbf{X}_i^0]_i = [(\bfx_i - \bar{\bfx}_i(KT))^{\top}, 0, 0]^{\top}$,
    where $\Delta \bfx_{ii} = \bfx_i - \bar{\bfx}_i(KT)$ and $\Delta \bfx_{ij} = \bfx_i - \bfx_j$.
\end{itemize}
The other networks are as follows: 
\begin{itemize}
    \item $\mathsf{MLP}$: for $\mathbf{R}$ and $\mathbf{J}$, $W=1$ and $(4\times n) \times (4\times 4\times n)$ parameters from $1$ unbaised layer; for $H$, $W=1$ and $(6\times n) \times (5\times 5\times n)$  parameters from $1$ unbaised layer. 
    \item $\mathsf{GNN}$: for $\mathbf{R}$ and $\mathbf{J}$, $W=1$ and $(4\times n) \times (4\times 4\times n)$ parameters from $1$ filter; for $H$, $W=1$ and $(6\times n) \times (5\times 5\times n)$  parameters from $1$ filter. 
    \item $\mathsf{GNNSA}$: for $\mathbf{R}$ and $\mathbf{J}$, $W=1$ and $(4\times n) \times (4\times 4\times n)$ parameters from $1$ filter; for $H$, $W=1$ and $(6\times n) \times (5\times 5\times n)$  parameters from $1$ filter; besides, $3 \times (4 \times 8) + (8\times 16)$ additional parameters from 
    three self-attention matrices and one self-attention vector. 
\end{itemize}
